EdgeShield: A Universal and Efficient Edge Computing Framework for Robust AI

The increasing prevalence of adversarial attacks on Artificial Intelligence (AI) systems has created a need for innovative security measures. However, the current methods of defending against these attacks often come with a high computing cost and require back-end processing, making real-time defense challenging. Fortunately, there have been remarkable advancements in edge-computing, which make it easier to deploy neural networks on edge devices. Building upon these advancements, we propose an edge framework design to enable universal and efficient detection of adversarial attacks. This framework incorporates an attention-based adversarial detection methodology and a lightweight detection network formation, making it suitable for a wide range of neural networks and can be deployed on edge devices. To assess the effectiveness of our proposed framework, we conducted evaluations on five neural networks. The results indicate an impressive 97.43% F-score can be achieved, demonstrating the framework's proficiency in detecting adversarial attacks. Moreover, our proposed framework also exhibits significantly reduced computing complexity and cost in comparison to previous detection methods. This aspect is particularly beneficial as it ensures that the defense mechanism can be efficiently implemented in real-time on-edge devices.

==> _ccs/ccs_concepts.tex <==
\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>10010520.10010553.10010562</concept_id>
  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010575.10010755</concept_id>
  <concept_desc>Computer systems organization~Redundancy</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010553.10010554</concept_id>
  <concept_desc>Computer systems organization~Robotics</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>10003033.10003083.10003095</concept_id>
  <concept_desc>Networks~Network reliability</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computer systems organization~Embedded systems}
\ccsdesc[300]{Computer systems organization~Redundancy}
\ccsdesc{Computer systems organization~Robotics}
\ccsdesc[100]{Networks~Network reliability}

==> _hid_del/0-Abstract_v1.tex <==
\begin{abstract}
The increasing prevalence of adversarial attacks on Artificial Intelligence (AI) systems has created a need for innovative security measures. 
However, the current methods of defending against these attacks often come with a high computing cost and require back-end processing, making real-time defense challenging.
Fortunately, there have been remarkable advancements in processing-in-memory (PIM) and near-sensor computing, which make it easier to deploy neural networks on edge devices. Building upon these advancements, we propose a PIM-based edge framework design to enable universal and efficient detection of adversarial attacks. 
This framework incorporates an attention-based adversarial detection methodology and a lightweight detection network formation, making it suitable for a wide range of neural networks and can be deployed on edge devices.
To assess the effectiveness of our proposed framework, we conducted evaluations on five neural networks. The results indicate an impressive 97.43\% F-score can be achieved, demonstrating the framework's proficiency in detecting adversarial attacks.
Moreover, our proposed framework also exhibits significantly reduced computing complexity and cost in comparison to previous detection methods. This aspect is particularly beneficial as it ensures that the defense mechanism can be efficiently implemented in real-time on edge devices.
\end{abstract}
%Our proposed solution showcases its effectiveness (achieving an F-score of 97.43\%) and broad applicability through extensive experiments, contributing a novel perspective to AI security efforts.


==> _hid_del/1-Introduction_v4.tex <==
\section{Introduction}
% 以下需要往边缘设备上靠，引出我们的动机
Edge devices and sensors usually run in a complex and noisy environment, where data are exposed to contamination with a high possibility. Combating these contamination usually caused by adversarial attacks in visual intelligent service requires neural networks with specific anti-interference optimization.
However, the extremely limited computing resources of edge devices severely limit the near-sensor deployment of high-workload robustness-strengthened neural networks.
%Although there have been some attempts to compute near-sensor convolutional neural networks, their compression and modification of neural network cause some damages to the models, among which vulnerability to adversarial attack is extraordinarily significant.
As a result, given security concerns in practical applications, the centralised approach is still the most commonly used in industry. 
In this mode, all the data collected by the sensor end will be transmitted to the central computing end regardless of perturbations and even attacks, and robustness-strengthened neural networks on the central computing end will shoulder the responsibility of fighting such adversarial attacks.
This creates redundant communication overhead and increases the workload on the computing center, which goes against the trend towards distributed and near-sensor computing.
%接下来一段的思路是阐述没有必要把被污染的数据传到back-end进行计算，既能减小communication开销，又能减小back-end的计算负载（这个怎么写一段需要想一下）
%接下来一段讲adversarial patches的一些特性（low-level feature， high activation），（说明现有的对抗adversarial patches的方法是怎么在我们的这个场景下失效的），以及adversarial patches的特性启发了near-sensor的AP detection

In recent years, emerging near-sensor computing architectures~\cite{du2015shidiannao,likamwa2016redeye, liu20191, ma2019analog} have been proposed to enhance the processing efficiency of edge devices. By moving specific processing closer to the sensor, these designs save data movements, storage, and bandwidth. 
Moreover, these architectures are easily integrated with the CMOS image sensor (CIS) module - a component of intelligent visual perception systems - allowing for always-on applications~\cite{ma2019analog}. Coupled with computing-in-memory (CIM) techniques~\cite{chi2016prime, yang201924, liu2020ns}, which conduct computation in analog domain, they effectively accelerate lightweight CNN processing on edge devices, making real-time processing possible.
% ShiDianNao hoists the CNN accelerator next to the CMOS or CDD sensor to entirely eliminate the DRAM accesses.
% RedEye pushes early processing of ConvNet into the analog domain that processes near sensors to reduce the workload of the analog readout. 
% Fei Qiao's group designs a visual perception chip that directly attaches the analog processing unit of BNN to CIS. This ADC-free architecture reaches ultra-low power consumption and high energy efficiency.
% In recent years, the substantial advancements in near-sensor computing have enhanced the capacity of edge devices to carry out lightweight neural network workloads. It can be easily integrated with prevalent CMOS image sensor (CIS) modules for always-on application to realize real-time data processing.
% One promising technology is the neuromorphic system with crossbar structures, which provides efficient implementations of near-sensor computing by simulating the biological brain's synapses, neurons, and kinetics.
%Using Ohm's law and Kirchhoff's law, the neuromorphic system can directly compute the matrix-vector multiplication (MVM) of neural networks in parallel without the need to digitize the outputs of sensors. 
% The emergence of advanced edge devices, such as resistive memory (ReRAM) devices~\cite{}, has further facilitated the efficient running of lightweight neural networks in the neuromorphic system. 
Exploring the potential of deploying a dedicated lightweight neural network at edge devices that utilizes near-sensor computing for real-time detection of visual attacks could prevent contaminated data from being transmitted to the back-end computing center. This novel strategy can effectively reduce redundant communication and computational load on the back-end, while also being a cost-effective solution for preventing visual attacks as it does not require custom defenses optimization for existing back-end neural networks that are already in use.


Adversarial patch attacks~\cite{eykholt2018robust, brown2017adversarial, karmon2018lavan} have emerged as an urgent threat among various adversial attacks~\cite{szegedy2013intriguing,goodfellow2014explaining,kurakin2018adversarial,moosavi2016deepfool,carlini2017adversarial,eykholt2018robust,brown2017adversarial,karmon2018lavan}. In this type of attack, a small yet carefully-crafted patch is placed randomly on an image obtained by the sensor. These patches have been proven to cause the back-end neural networks to generate abnormal activation layer by layer~\cite{yu2021defending}, which weakens the authentic features of the original image and deceives the back-end system into misidentifying the image. The simplicity of training and the low-cost deployment of such attacks makes them attractive to malicious actors seeking vulnerabilities in visual intelligence systems. As a result, the trustworthiness and reliability of these systems are compromised.
%, including but not limited to facial recognition, object detection, autonomous driving, and surveillance systems
Thus, it is imperative to detect adversarial patch attacks.

Many works have proposed solutions to tackle the security issue of back-end intelligence system caused by adversarial patch attacks. However, none of these solutions are currently applicable to edge devices. For instance, Digital Watermarking (DW)~\cite{hayes2018visible} and Local Gradient Smoothing (LGS)~\cite{naseer2019local} have been proposed as patch removal techniques that locate and either erase or mask patches. %However, they perform poorly in patch detection and often compromise significant parts of the clean image. 
LanCe~\cite{xu2020lance} defined Input Semantic Inconsistency for patch detection,
%, but its computation is too complicated and requires the prediction class of the data, limiting its applicability to post-prediction correction. 
while Yu~\cite{yu2021defending} introduced Feature Norm Clipping (FNC) layer between layers of the model and defined the Incremental Feature Norm Ratio (IFNR) to assess the effectiveness of FNC layers.
%, but its clipping strategy still damages clean images. Moreover, calculating IFNR and introducing FNC layers with the L-2 norm increase the algorithm's complexity and the neural network's computational overhead. 
%In summary, 
These approaches cannot be implemented on edge devices as their patch detection or removal depends on specifically optimized neural networks for the original back-end models, which is both time-consuming and resource-intensive. 

\begin{figure*}[!t]
  \vspace{-3mm}
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=7in, height=3.5in]{_fig/Fig1.pdf}
  \caption{The framework of our proposed method.}
  \label{fig:Fig1}
  \vspace{-5mm}
  % \Description{}
\end{figure*}

In contrast to previous methods that require custom optimization of the back-end neural networks, we propose the first framework that exploits edge devices to develop an effective and cost-efficient method to enhance the security of visual intelligence systems. As shown in Fig.~\ref{fig:Fig1}, our approach employs a universal lightweight neural network embedded in edge devices to detect various types of adversarial patches by identifying abnormal values in the attention map. The detection model is lightweight, making it resource-efficient and well-supported for edge deployment. Combing computing in memory technology can optimize resource utilization and enables real-time attack detection. With this universal detection model, there is no need to enhance and re-deploy the back-end neural networks that are already widely deployed in the industry. 
% The requirement of adjusting edge-built model to match the back-end system is also eliminated. 
By preventing contaminated data from being uploaded, our framework reduces communication bandwidth, enhances the accuracy and reduce workload of the back-end intelligence system. 
This work provides a promising solution to the issue of AI security.

% Our framework is applicable to a wide range of visual intelligence systems and can help improve the overall security and efficiency of these systems. 

% 再加点实验结果，精度，计算量等。
% In summary, the method proposed in this paper has greatly reduced computational and deployment costs for adversarial patches detection and its application field is wide. The experiment shows its F1-score can reach 97\% in the detection of all kinds of adversarial patches.


==> _hid_del/2-Background_v3.tex <==
\section{Background}
\subsection{AI Trustworthiness}
% 简要介绍深度神经网络的发展，带出常被攻击的经典CNN模型,即为后文实验用的 thread model
% 介绍adversarial patch, 与传统 adversarial attack 进行区分，以及由于adversarial patch的训练和部署成本低，应用广泛且难以预防，本文关注对adversarial patch 的预防。
The increasing advancements in deep convolutional neural networks (CNNs) have led to their widespread adoption in various visual intelligence systems, including but not limited to facial recognition, object detection, autonomous driving, and surveillance systems. Typical and powerful CNNs, such as VGG-16~\cite{simonyan2014very}, ResNet-50~\cite{he2016deep}, MobileNet-V2~\cite{sandler2018mobilenetv2}, Inception-V3~\cite{szegedy2016rethinking}, and ResNet-101~\cite{he2016deep} have large scales and complex structures. However, these models are vulnerable to visual attacks, particularly adversarial patch attacks, where a small universal patch trained on a limited dataset is attached to the model's inputs~\cite{brown2017adversarial}. Patches trained against one model exhibit varying levels of transferability to other models. Thus, this paper focuses on developing a universal and efficient method for detecting all adversarial patches trained against varying models. 

Although many approaches have been proposed to address this issue, they all suffer from certain limitations. DW~\cite{hayes2018visible} and LGS~\cite{xu2020lance} perform poorly in patch detection and can compromise significant parts of the clean image. LanCe~\cite{xu2020lance} detects inconsistencies between the output of the model's last layer and the synthesized pattern of the predicted category. However, this approach requires computing thresholds for synthesized patterns of each category, which can be time-consuming. Furthermore, the computation of the inconsistency requires knowledge of the predicted class of the output, limiting its use to post-prediction correction.
Yu et al.~\cite{yu2021defending} proposed adding FNC layers to clip the outputs of specific layers in the model. They also defined the IFNR metric to demonstrate that the impact of patches on IFNR values is mitigated after processing the outputs of selected layers with FNC layers. The FNC clipping strategy involves replacing the values of all points in the feature map where the L-2 norm is greater than the mean. However, this clipping strategy also affects the larger values in the feature map of clean images that contribute more to the classifier's output, resulting in noticeable damage to the clean images. Moreover, the computation of IFNR and the introduction of FNC layers increase the algorithm's complexity and the neural network's computational overhead.

%To analyze the impact of adversarial patches on these models, we trained patches against each model with 2000 images from ImageNet and then evaluate the top-1 accuracy of each model under path attacks, as presented in Table 1. It showed that adversarial patch have varying degrees of transferability. VGG-16 and Inception-V3 are more susceptible to patch attacks, while MoblieNet-V2 is relatively robust. This provides a possible explanation for the higher transferability of the patch trained against MobileNet-V2 (AdvP-MobileNetV2) and its relative difficulty to detect, as demonstrated in subsequent experiments (table 2 and table 3).

\subsection{Near-Sensor Computing}
% 介绍部分工作是怎么做的，以及ReRAM用于neuromorphic computing
% 说明将检测移到edge端的必要性
The emerging architectures of near-sensor computing provide a novel avenue to tackle the issue of AI trustworthiness. Near-sensor computing is a rapidly evolving field within edge computing that seeks to bring computation closer to the data source by embedding processing capabilities near sensor sides. 
% This paradigm dramatically reduces data movement, cutting down on energy consumption and latency, thus making real-time visual attacks detection feasible.

ShiDianNao~\cite{du2015shidiannao} hoists the CNN accelerator next to the CMOS or CDD sensor to entirely eliminate the DRAM accesses.
RedEye~\cite{likamwa2016redeye} pushes early processing of ConvNet into the analog domain that processes near sensors to reduce the workload of the analog readout.
Fei Qiao's group designs a visual perception chip that directly attaches the analog processing unit of BNN to CIS~\cite{liu20191}. 
This architecture design eliminates the need for ADC and conventional analog buffers, reaching ultra-low power consumption and high energy efficiency. 
% This ADC-free architecture reaches ultra-low power consumption and high energy efficiency.
% Subsequently, they propose an analog-memoryless near-sensor computing architecture that shifts the correlating-double-sampling (CDS) operation to the Computation Module~\cite{ma2019analog}. This move leads to a reduction in hardware overhead and an enhancement in energy efficiency.
NS-CIM~\cite{liu2020ns} integrates near-sensor computing architecture with the computing-in-memory paradigm to process sensory signals locally, significantly cutting down on data conversion and movement.

\begin{figure}[t]
  \vspace{-3mm}
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.0cm}
  \centering
  \includegraphics[width=\linewidth]{_fig/Fig2.pdf}
  \caption{Samples perturbed by adversarial patch at different locations.}
  \label{fig:Fig2}
  \vspace{-5mm}
  % \Description{}
\end{figure}

Moving visual attack detection to the edge via near-sensor computing is significant. First, it reduces latency and energy consumption, as the need to transfer raw data to the cloud for processing is eliminated. Second, on-device detection enhances security as it prevent data may include Trojan attacks from uploading. As such, leveraging near-sensor computing with CIM technology in visual attack detection presents a practical, efficient, and robust approach for improving the security of real-world AI applications.





==> _hid_del/3-Method_v3.tex <==
\section{Designed Methodology}
% 1. 附上部署的框架图（类似EARLIN的整合图3：collaborative inference）以及detection 部分的框架图(类似EARLIN的图1)，介绍模型包含哪几部分(detection、classify)

In this section, we will introduce our method for adversarial attacks detection on edge devices. As shown in Fig.~\ref{fig:Fig1}, the framework of our work consists of two parts: detection and inference. The detection is deployed on an edge device that collects inputs through sensors. That stage will make use of the shallow layers output of VGG-16. After detection, only if the input is detected as a clean image will it be uploaded to the back-end computing centre for inference. The inference part is a full deep CNN deployed on the server, proven excellent in classification, such as VGG-16, ResNet-101, Inception-V3, etc. Note that we only upload the original image instead of the intermediate output of VGG-16 to reduce the bandwidth pressure during the upload.

\subsection{Attention-based Method for Attacks Detection}
% 1. 介绍attention map，与传统的 attention 机制（attention 因子是模型在训练过程中需要进行学习的参数）进行区分（需要补充）
%2. 介绍本文Attention Map的计算公式，以及如何用于检测
It is observed that adversarial patches mislead classifier result by causing some signiﬁcant abnormalities that overwhelm the original decision portion in the last convolution activation map~\cite{xu2020lance,yu2021defending}. Instead of introducing complex calculations of L-2 norm or inconsistency, we propose using the attention map generated from the activation map of a particular layer for attack detection. Each point in attention map is defined as Eq. 1.
\begin{equation}
A_{T}(F,h,w) = \frac{1}{C} \sum_{i}^{C}F_{h,w}(i)
\end{equation}
$F\in \mathbb{R}^{C\ast H\ast W}$ is the activation map for a certain layer in the model. $F_{h,w}(i)$ represents the activation value of the $i^{th}$ channel at coordinates \begin{math} (h,w)\end{math} in activation map. The attention map is calculated by taking the mean of the activation map along the channel dimension C. Then, we would obtain an attention map $A_{T}(F)$ of size $H\ast W$ for the activation map $F$.

The attention maps generated by a specific activation layer of VGG-16 show significant differences between clean and perturbed inputs, as demonstrated in Fig.~\ref{fig:Fig2}. Specifically, the attention map for perturbed input exhibits a higher focus on the patch region. Inspired by this observation, we suggest that the maximum value in the attention map contains the most salient features, and we define it as the $I_{r}$ indicator:
\begin{equation}
I_{r}(A_{T}) = \max A_{T}(F,h,w)
\end{equation}

The following will explain how to leverage attention maps for attack detection. We computed $I_{r}$ values for 20,000 perturbed images and their corresponding clean images from ImageNet dataset~\cite{russakovsky2015imagenet} on a specific convolution layer of VGG-16. The $I_{r}$ distributions for clean and perturbed samples were found to be well separated, enabling us to determine a threshold value $\Theta$ to distinguish them with a certain level of confidence $p$, using only the $I_{r}$ values from clean samples.
\begin{equation}
p = \frac{\sum_{A_{T}\in A_{T}^{clean}}\mathbb I(I_{r}(A_{T})\leq \Theta)}{|A_{T}^{clean}|}
\end{equation}
$A_{T}^{clean}$ represents a set of attention maps generated from numerous clean samples. $|A_{T}^{clean}|$ indicates the number of elements in $A_{T}^{clean}$, also the number of clean samples. The symbol $\mathbb I()$ is an indicator function that returns $1$ if the condition in parentheses is True, and $0$ otherwise. Given a confidence level $p$ (usually set to 0.95), we calculate a threshold value $\Theta$ such that $p$ fraction of the clean samples satisfy $I_{r}(A_{T})\leq \Theta$. It is worth noting that our method for computing $\Theta$ does not require any exposure to perturbed samples.

\begin{figure*}[!t]
  \vspace{-3mm}
  \setlength{\abovecaptionskip}{1.3mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=\textwidth,height=1.4in]{_fig/Fig3.pdf}
  \caption{Distributions of $I_{r}$ indicators at different layers of VGG-16 on ImageNet.}
  \label{fig:Fig3}
  \vspace{-5mm}
  % \Description{}
\end{figure*}

% \begin{figure*}[!t]
%   % \vspace{-3mm}
%   \setlength{\abovecaptionskip}{1.4mm}
%   \setlength{\belowcaptionskip}{-0.cm}
%   \centering
%   \includegraphics[width=0.85\textwidth,height=2.5in]{_fig/Fig5.pdf}
%   \caption{The Process of calculating threshold and of experiments for detector evaluation.}
%   \label{fig:Fig5}
%   \vspace{-5mm}
%   % \Description{}
% \end{figure*}

Finally, the detection of attacks can be formulated as Eq. 4.
\begin{equation}
\mathcal{D}(x) = 
\begin{cases}
1\ \ (perturbed), \quad {if} \ \ {I_{r}(A_{T})>\Theta},\\
0\ \ (clean), \quad {otherwise.}
\end{cases}
\end{equation}
For an input sample $x$, we obtain its attention map $A_{T}$ and corresponding $I_{r}$ indicator on a specific convolution layer of VGG-16. Our detection model is based on the cascaded architecture from the first layer up to the specific layer of VGG-16. We would lilke to note that all models used in our study, including VGG-16, ResNet-101, Inception-V3, etc., do not require any additional training since we obtained their weights from official sources.

\subsection{Detection Layer Selection}


In this section, we will discuss the selection of a specific convolution layer for attack detection in our proposed method. We collected $I_{r}$ indicators on various convolution layers of VGG-16 and plotted their frequency histograms as shown in Fig.~\ref{fig:Fig3}. The results demonstrate that the distributions of clean and perturbed $I_{r}$ are more separate in shallower layers. Perhaps, this observation can be interpreted based on the principle of convolution operation and adversarial attacks. Adversarial attacks aim to draw more attention to the perturbed areas of an image, which often results in increasing values in attention maps. So the $I_{r}$ indicator, maximum value in attention map, is the most sensitive to this impact. As the convolution layer becomes deeper, the impact of the adversarial attack is propagated to more pixel points in the feature map. This leads to an increase in the number of points with higher values in the attention map, but the magnitude of the increase decreases. Consequently, the impact of individual values weakens, while the overall impact of the combined values increases.

After analyzing the results mentioned above, we have confirmed that $I_{r}$ is a highly precise indicator for detecting attacks in shallow convolution layers. Consequently, selecting such layers as the detection layer can considerably decrease hardware costs during implementation. Furthermore, our approach enables real-time attack detection by eliminating the requirement of running the complete inference of deep CNNs for detection, which is made possible by choosing shallow convolution layers as the detection layer. Specifically, we recommend choosing the 2nd convolution layer of VGG-16 as the detection layer, as demonstrated in the subsequent experiments.

% \begin{figure*}[!b]
%   \vspace{3mm}
%   \setlength{\abovecaptionskip}{1.4mm}
%   \setlength{\belowcaptionskip}{-0.cm}
%   \centering
%   \includegraphics[width=\textwidth,height=1.4in]{_fig/Fig4.pdf}
%   \caption{Distributions of $I_{c}$ indicators at different layers of VGG-16 on ImageNet.}
%   \label{fig:Fig4}
%   \vspace{-3mm}
%   % \Description{}
% \end{figure*}


%We used the original adversarial patch method~\cite{brown2017adversarial} to train an adversarial patch against VGG-16~\cite{simonyan2014very} with small part samples (2000) from Imagenet~\cite{russakovsky2015imagenet}. This patch with a size of only 6\% of the original image dropped the top-1 accuracy of VGG-16 to 1.3\% on Imagenet. 

%At first, we observed its influence on the attention map at the last convolution layer. Fig.~\ref{fig:Fig2} shows two examples that the original image and perturbed will get into huge differences at the place of the patch, where the perturbed will be significantly higher in values. We further selected different layers to analyze the influence of adversarial patch attacks. We found that the difference shows up earlier than we thought. That inspired us to take advantage of this early difference for detection. So we are supposed to define an indicator to represent the whole attention map that will better maximize the difference. As shown in Fig.~\ref{fig:Fig2}, the values range of a attention map is relatively narrow before the attack. But the patch considerably increased the upper limit of the range at all layers. So we will take the upper limit of range as the indicator for one attention map, which defined by:

% In the upcoming section, we will present our experimental methodology and analyze the obtained results. our experiments were conducted to investigate which deep CNNs are suitable for reconfigurable detection of various adversarial attacks, utilizing their shallow layers as a unified model for detection. Moreover, We intend to determine the optimal shallow layer for detection and assess the implementation cost.

==> _hid_del/4-Experiment_v3.tex <==
\section{Experiment and Evaluation}
% The experiment details are presented in Fig.~\ref{fig:Fig5}. 
% We perform a 4:6 stratified random sampling of the ImageNet dataset~\cite{russakovsky2015imagenet} to obtain the analysis dataset (40\%) and the test dataset (60\%). Half of the test dataset is randomly attacked to generate a balanced dataset of positive (attacked images) and negative (clean images) samples. Using the analysis dataset, we calculate the threshold $\Theta$ of $I_{r}$ indicators, which we utilized to detect the test dataset.

\subsection{Experiment Setup}
% 介绍模型的评价指标P,R,F
% 总的实验框架图，分为分析和测试两步Fig. 7.

% \textbf{Evaluation Metric:} 
% Unlike previous research, which evaluated detection models solely based on accuracy using only attacked images as input data, our approach is comprehensively evaluated using commonly used classifier metrics, including precision ($P$), recall ($R$), and F-score ($F$). These metrics require the model's input dataset to consist of both positive and negative samples, allowing us to account for the possibility of falsely classifying clean images as attacked.

\textbf{Detection Layer:} The shallow layers used to obtain $I_{r}$ indicators are taken from VGG-16, but other classic models such as ResNet-50, MobileNet-V3, and others can also be used. The selection of detector models and layers will be discussed in the Ablation Studies section.

\input{_tab/tab1_v2}

\textbf{Attacks Training:} We utilized the original adversarial patch attacks developed by Brown et al.~\cite{brown2017adversarial} to train diverse adversarial patches, which occupy only 6\% of the original image size, against several typical deep CNNs, respectively. We extracted a small sample of 2000 images from ImageNet to train these patches. As presented in Table~\ref{tab:table1}, the top-1 accuracy of the corresponding threat models was reduced to the range of 0.83\% to 33.98\% on Imagenet.



\subsection{Effectiveness of Detection} % Performance of Detection
% 简单介绍针对各种thread models 在Imagenet数据集训练的patch
% vgg16模型的浅层用于检测各种patch，列出实验结果和图，以及模型求出的参数：threshold值
% 实验结果可以和Lance中detection部分进行比较
% 说明在模型应对针对不同网络的patch时，检测层无需做出变更，甚至threshold值都不需要改变
%gpu cost 
From Table~\ref{tab:table1} we observe that adversarial patches cause varying degrees of Top-1 accuracy degradation in classical models, with VGG-16 being the most vulnerable to patch attacks, while MoblieNet-V2 is relatively robust and difficult to attack. We aim to build a unified model to detect all threat models' adversarial patches. 

\input{_tab/tab2}
\input{_tab/tab3}

To accomplish this, we leverage the shallow layers of VGG16 as a unified model to derive the $I_{r}$ indicator and calculate $\Theta$. The detection results, as shown in Table~\ref{tab:table2}, reveal that the second convolutional layer of VGG-16 emerges as the optimal choice for the detection layer, i.e., utilizing the $I_{r}$ indicator, derived from the feature map after the first two layers, offers the best performance in attack detection. All attacked inputs can be correctly identified (R=100\%), and about 95\% of clean images are guaranteed not to be falsely identified as attacked (P$\approx$95\%), with an F-score of at least 97.42\%. The results also suggest that one of the adversarial patches, called Advp-MobileNetV2, which is trained on the robust MobileNet-V2, tends to be more aggressive and exhibits higher cross-model transferability, making it challenging to detect. In scenarios where the edge device is grappling with extreme resource constraints, deploying only the first layer of VGG-16 could still be a viable option. It retains an F-score of at least 87.91\%, even when subjected to the Advp-MoblieNetV2 attack.

% \input{_tab/tab2}

\textbf{Ablation Studies:} We conducted additional experiments to investigate the effectiveness of using shallow layers of different models as a unified model for detection. The results, presented in Table~\ref{tab:table3}, confirm that the detection of Advp-MoblieNetV2 remains the most challenging among all the threat models' adversarial patches, as we previously discussed. In the absence of Advp-MoblieNetV2, it can be concluded that the first convolution layers of all models are suitable for detection, with the F-score reaching at least 92.17\%. However, when considering Advp-MoblieNetV2, only the first convolution layers of ResNet-50 and MobileNet-V2 are additional options as unified models for detection, with an F-score of at least 80.91\%. Combining the results from Table~\ref{tab:table2} and Table~\ref{tab:table3}, we can state that the second layer of VGG-16 is the best-performing unified model for detecting all adversarial patches trained from different threat models. The F-score achieved by this model is at least 97.42\%, surpassing the previous state-of-the-art performance achieved by LanCe~\cite{xu2020lance}. LanCe attained an accuracy of 91\% but did not consider the possibility of falsely classifying clean images as attacked.

% \textbf{Interpretation of Results:} The optimal choice obtained from the experimental results may be attributed to the fact that VGG-16 is the most vulnerable model among all the threat models, as shown in Table~\ref{tab:table1}. This vulnerability allows patches trained by other threat models to possess some level of transferability to attack VGG-16. As a result, the shallow layers of VGG-16 demonstrate sensitivity to all patches and exhibit the capability to capture pertinent features that indicate the presence of adversarial patches.

%The reason for this result may be that the VGG-16 is the most vulnerable among all the threat models, so all patches trained by other models have some level of transferability to attack VGG-16. As a result, the shallow layers of VGG-16 are sensitive to all patches and have the ability to capture relevant features indicative of adversarial patches.

%This happens may because from the adversarial attacks training, we can see the VGG-16 is the most vulnerable model




%\subsection{Memory and Operation Complexity}
% 将以上各种patch，换其他模型的浅层进行检测, 列出实验结果和图，以及不同的threshold值
% 确定哪个模型的浅层更适合作为统一的检测模型
% 这个确定的过程中，不应该只看实验结果，在实验结果差不多的情况下，应选择浅层结构更简单的模型
% 选择的指导建议
% 浅层结构的复杂度评估：
% 1.计算单元的数量 
% 2.计算过程中需要store并transfer的中间结果数量 
% 3.MADD,FLOPS
% 1.可以找到模型
% 2.实验指导意义
%In order to guide the layer and model selection for patch detection, we analyzed the information of each model shallow layer, as shown in Table~\ref{tab:table4}.
%\input{_tab/tab4}
\subsection{Computational Cost}
In this section, we aim to benchmark the computational cost introduced by our proposed method against those incurred by previous methods. 
% The computational cost comparsion will not include the inference of CNNs as each method have. 
% The computational cost directly influences the speed and efficiency of these methods. Our comparisons will focus on two aspects and all comparisons will conduct with different deep CNN models. 
% Note that the comparison only considers the cost introduced by these methods，excluding the original neural network computation.
Firstly, we evaluate the preliminary computations required before the methods can be deployed, 
% we need consider the preparatory work required before the deployment of methods, 
including the calculation of thresholds in ours and LanCe's, and verify process (calculation of FNC and IFNR) in Yu's. 
LanCe's detection process comprises three stages: 2D Fast Fourier Transform (2D-FFT), Class Activation Mapping (CAM) and Jaccard Similarity Coefﬁcient (JSC) calculations. Given C classes with N examples each, each stage executes $ CN$ times to acquire the necessary thresholds.
% The CAM calculation involves ADD operations on the final feature map (FFM). 
% of size $k\times h\times w$. 
% For an image of dimensions $H\times W$, the 2D-FFT calculation involves $(HW\log(W) + HW\log(H))$ multiplications and equivalent ADD operations. The JSC calculation requires logical AND or OR operations executed $hw\log(hw)$ times.
In Yu's approach, the computations comprise the FNC layers, introduced at each cascaded module (examples include introducing the FNC layer after each convolution block in VGG-16), and INFR, which necessitates calculating the L-2 norm of the feature map. To simplify comparison, we assume that the FNC layer is added only to the initial cascaded module.
% they calculate the INFR for each pair of adversarial and clean images that involve computing norm maps and introduce FNC layers to the feature maps of each cascaded module (e.g. Convolution block for VGG-16). For simplicity in comparison, we assume they add the FNC layer only to the first cascaded module.
% In Yu's methodology, the calculation of the IFNR for each pair of adversarial and clean images involves generating norm maps from the final feature maps, supplemented by four SUB/ADD and comparison operations within these map dimensions. Additionally, they introduce FNC layers to the feature maps of each cascaded module (e.g. Convolution block for VGG-16). For simplicity in comparison, we assume they add the FNC layer only to the first cascaded module.
% Generating the norm map for a $k\times h\times w$ dimensional feature map requires $khw$ multiplications and an equal number of ADD operations. 
Our method, however, focuses computationally on generating the attention map from the feature map of the second convolution layer, i.e., the first convolution block of VGG-16. We then identify the maximum value within this attention map.
% Indeed, we are assuming that the number of examples N, used in our method to compute thresholds and in Yu's method to calculate IFNRs, is the same. This assumption is based on the equal number of examples used in LanCe to calculate thresholds for each class. 
% \input{_tab/table5_v2}
% The comparison of computational cost during the threshold calculation and verify stage of these methods is presented in Table~\ref{tab:table5}. The results suggest that our method demands considerably fewer computational resources during this stage than the LanCe and Yu approaches. More specifically, ours involves only ADD/SUB and comparison operations, which are less complex at the hardware level and less demanding in processing power than the multiplication operations necessitated by the other two methods.
% Because multiplication requires a series of shift and ADD operations, while ADD operation can usually be completed in one processor cycle.
% Thus, our approach provides a more computationally efficient solution for practical applications.
% \input{_tab/table6}
% \input{_tab/table7}
Secondly, we assess the computational costs during the actual implementation stages of these methods. During this phase, Yu's method emphasizes the computation of FNC layers, while LanCe's and Ours execute the same steps as in the former stage for each sample.


\input{_tab/table5_v2}
The comparison is illustrated in Table~\ref{tab:table5}, where all computations mentioned above can be dissected into four basic types of hardware operations. Our method stands out by significantly reducing the computational burden, primarily by avoiding the expensive multiplication operations. Moreover, our method exhibits superior efficiency by requiring only a single register to store the threshold, a sharp contrast to LanCe's requirement of 1000 registers for multiple thresholds. This efficiency not only conserves memory space but also simplifies system implementation and minimizes overall complexity. 
Thereby, our method is particularly suitable for deployment in resource-constrained environments, such as edge devices.
% Table~\ref{tab:table7} provides a summary of the computational operations involved throughout all stages.
% Thereby, our method proves highly efficient due to its lower computational cost and reduced need for register storage, making it particularly suitable for deployment in resource-constrained environments, such as edge devices.

% our approach emerges as a highly efficient solution, particularly apt for deployment in resource-constrained settings, such as edge devices.
% As a result, our approach proves highly efficient and well-suited for deployment in resource-constrained environments, such as edge devices.



==> _hid_del/5-Conclusion_v1.tex <==
\section{Conclusion}
% 对以上的实验结果进行总结，结合实验结果说明我们方法的优点
% 对进一步优化的展望：为部署到边缘设备中，进一步对用于detection的模型浅层进行简化
% 未来会尝试在边缘设备上进行部署和验证
In this paper, we proposed a highly adaptive and universal edge AI framework for robust visual intelligence. The framework leverages the attention map derived from the shallow layers' feature map of a deep CNN to effectively identify a broad spectrum of visual attacks. The experiments conducted in this study have demonstrated the effectiveness and universal applicability of our approach, achieving an F-score of at least 97.4\% in detecting various attacks. Furthermore, our method offers several advantages when implemented on edge devices. It requires less computational cost and memory for registers, and eschews complex multiplication. These characteristics make it highly suitable for resource-constrained environments. Additionally, our approach does not require any knowledge of or modifications to the back-end AI model, enabling seamless integration with widely-deployed industrial AI models. 
% This highlights the adaptability of our work.

% Overall, our framework showcases the adaptability and universality of edge AI solutions for robust visual intelligence. We believe that our work contributes to the advancement of the field and opens up opportunities for real-world applications in diverse domains.



% Our framework leverages the attention map, derived from the shallow layers' feature map of a deep CNN, to effectively identify a broad spectrum of visual attacks. Experiments showcase the effectiveness and broad applicability of our approach, as it achieves an F-score of at least 97.4\% in detecting various attacks. Additionally, our method, which requires less computational cost and eschews complex multiplication, is particularly advantageous when implemented on edge devices. Furthermore, implementing our approach necessitates no specific knowledge of the back-end AI model, suggesting that even widely-deployed industrial AI models require no modifications for edge detection. This feature further emphasizes the adaptability of our framework.




% In this paper, we proposed a universal and elastic edge AI framework for robust visual intelligence. This framework utilize the attention map generated from feature map of deep CNN's shallow layers to detect various visual attacks. The experiment shows that our approach can achieve F-score at least 97.4\%. With the efficiency to detect 100\% attacked images and guarantee not misidentify 95\% clean images as perturbed. 

==> _his/0-Abstract_v1.tex <==
\begin{abstract}
The increasing prevalence of adversarial attacks on Artificial Intelligence (AI) systems has created a need for innovative security measures. 
However, the current methods of defending against these attacks often come with a high computing cost and require back-end processing, making real-time defense challenging.
Fortunately, there have been remarkable advancements in computing-in-memory (CIM) and near-sensor computing, which make it easier to deploy neural networks on edge devices. Building upon these advancements, we propose a PIM-based edge framework design to enable universal and efficient detection of adversarial attacks. 
This framework incorporates an attention-based adversarial detection methodology and a lightweight detection network formation, making it suitable for a wide range of neural networks and can be deployed on edge devices.
To assess the effectiveness of our proposed framework, we conducted evaluations on five neural networks. The results indicate an impressive 97.43\% F-score can be achieved, demonstrating the framework's proficiency in detecting adversarial attacks.
Moreover, our proposed framework also exhibits significantly reduced computing complexity and cost in comparison to previous detection methods. This aspect is particularly beneficial as it ensures that the defense mechanism can be efficiently implemented in real-time on-edge devices.
\end{abstract}
%Our proposed solution showcases its effectiveness (achieving an F-score of 97.43\%) and broad applicability through extensive experiments, contributing a novel perspective to AI security efforts.


==> _his/1-Introduction_v1.tex <==
\section{Introduction}
% 以下需要往边缘设备上靠，引出我们的动机
Deep Convolutional Neural Networks (CNNs) are widely deployed in the physical world because of their promising performance on computer vision tasks. Their application scenarios involve numerous security areas, such as face recognition, assisted driving, medical image diagnosis, etc. However, CNNs are found vulnerable to adversarial attacks~\cite{szegedy2013intriguing,goodfellow2014explaining,kurakin2018adversarial,moosavi2016deepfool,carlini2017adversarial,eykholt2018robust,brown2017adversarial,karmon2018lavan}, where purposefully lightly perturbing a pretty small portion of pixels of the image to fool the model (taken as a threat model) make a wrong decision, causing heavy security risks for CNNs applications. Among all adversarial attacks, adversarial patches~\cite{eykholt2018robust,brown2017adversarial,karmon2018lavan} are the most popular for attackers to apply, as they are more effective and cost-efficient than conventional attacks.
% the adversarial patches~\cite{eykholt2018robust, brown2017adversarial, karmon2018lavan} are the most prevalent as they are more efficient and cost-saving than conventional adversarial attacks. 
This paper will focus on the detection of adversarial patches. In the realistic industry scene, deep CNNs are normally deployed on a server (e.g., cloud) because of the requisition of several billion computing operations. Resource-constrained edge devices usually upload inputs to the server to make inferences. If adversarial patches could be detected with edge devices, that could certainly save communication and computation workloads by blocking those attacked inputs from uploading. This Inspired us to find an efficient way to detect adversarial patches early before they are uploaded from edge devices.

% 以下修改需要往patch detection 方向说，挑defence中的detection部分解说
Many approaches have been proposed to solve this security issue raised by the adversarial patch attack, but they both suffer several limitations. Digital Watermarking (DW)~\cite{hayes2018visible}, Local Gradient Smoothing (LGS)~\cite{naseer2019local} defense attacks by erasing or soft masking patches after locating them. They perform poorly in detection and usually weaken significant parts of the clean image. LanCe~\cite{xu2020lance} defines Input Semantic Inconsistency to calculate the difference between the input image and its predicted class original images for patches detection. However, the computation is too complicated and requires the prediction class of the model, which means it is impossible to detect patches early at resource-constrained edge devices. That increases the computational and time costs. Yu~\cite{yu2021defending} introduces Feature Norm Clipping (FNC) between layers of the model and defines the Incremental Feature Norm Ratio (IFNR) to analyze the impact of FNC layers. Although it gets some improvements on previous works, its clipping strategy is still time-consuming and the layers for every clean image are also been clipped. It is difficult to calculate the IFNR and doing clipping for they introduced L-2 norm. Besides, the addition of FNC layers will also increases the complication of deep CNNs.

In this paper, we proposed a framework for adversarial patches detection early on edge devices. At first, we analyze the effects of adversarial patches on the attention maps of each layer output of several CNN models. Then, we visualize and quantify these effects and propose a method for adversarial patches detection using the early layer's output of a unified model. Our method has several advantages over previous works and we summarize as follows:

\begin{itemize}[itemsep=2pt,topsep=0pt,parsep=0pt,listparindent=0pt]
\item Our detection model makes use of the early layers of a typical CNN model and we needn't redesign and retrain any model; 

\item The number of computing units we introduce for adversarial patch detection after early layers of CNNs is limited. The operations such as sum and comparison for detection are simple as well. 

\item When facing different adversarial patches trained from different threat models, we have a unified model to detect the patches. That means we needn't modify our model with the patch changing for different threat models. 

% \item When our model is applied to a different domain,  it means our model will face adversarial patches trained from another domain dataset. The only requirement for our model is to switch the threshold of detection, which is already prepared before the model is deployed. 

\item Our model can be deployed on edge devices to intercept input images with patch attacks for various heavy deep learning models on the cloud. Thus, we can improve the accuracy of subsequent models and avoid the consumption of uploading bandwidth by perturbed images. Meanwhile, no alterations are required for the classifiers that are already industrially deployed in servers. That will avoid the cost of redeployment.
\end{itemize}

In summary, the method proposed in this paper has greatly reduced computational and deployment costs for adversarial patches detection and its application field is wide. The experiment shows its F1-score can reach 97\% in the detection of all kinds of adversarial patches.



==> _his/1-Introduction_v2.tex <==
\section{Introduction}
% 以下需要往边缘设备上靠，引出我们的动机
Deep Convolutional Neural Networks (CNNs) are widely deployed in the physical world because of their promising performance on computer vision tasks. The application scenarios involve face recognition, assisted driving, medical image diagnosis, etc. The inference stage of deep CNNs tends to require several billion computing neurons, making it difficult to apply on edge devices, which are constrained in computation, memory, and storage. The feasible solution is to transfer the large amount of raw data acquired by sensors to back-end devices, such as clustered local servers or cloud-based computing systems, where the resources are sufficient for data processing and model inference. This is computing architecture generally adopted in the actual industry. But it raises other issues of energy consumption, communication bandwidth and security. With the development of edge- and sensor-computing, it is possible to transfer low-level data processing workload (noise suppression, edge extraction, contrast enhancement, etc.) to front-end devices, such as edge devices near sensor or even in sensor~\cite{zhou2020near}. The front-end devices play a role to process, save, upload data, and receive outputs of predictors from back-end devices. That efficient data processing strategy reduces redundant raw-data communication between sensors and back-end devices. However, edge devices and sensors usually run in a complex and noisy environment, where let data are exposed to contamination with a high possibility. It offers opportunities for attackers to fool the models. For example, adversarial attacks~\cite{szegedy2013intriguing,goodfellow2014explaining,kurakin2018adversarial,moosavi2016deepfool,carlini2017adversarial,eykholt2018robust,brown2017adversarial,karmon2018lavan} deceive models into false predictions by perturbing a tiny small portion of pixels of the image, causing severe security risks for deep CNNs applications.
In particular, adversarial patches~\cite{eykholt2018robust,brown2017adversarial,karmon2018lavan} are widely used in the physical world by attackers, as they are more effective and cost-efficient. Therefore, it is urgent to monitor data for uploading and tackle such trustworthiness problems for deep CNNs. If the data quality can be guaranteed before uploading, it will improve the accuracy of models and save bandwidth of polluted data transmission.

Many works have proposed to tackle the security issue of deep CNNs applications. Works to defend against attacks of adversarial patches, for instance, Digital Watermarking (DW)~\cite{hayes2018visible} and Local Gradient Smoothing (LGS)~\cite{naseer2019local}. They erase or soft mask patches after locating patches. But they perform poorly in patch detection and usually weaken significant parts of the clean image. LanCe~\cite{xu2020lance} defines Input Semantic Inconsistency for patch detection. However, its computation is too complicated and requires the prediction class of the data, which means they can only correct the mistake prediction after it happens. Yu~\cite{yu2021defending} introduces Feature Norm Clipping (FNC) between layers of the model and defines the Incremental Feature Norm Ratio (IFNR) to prove the FNC layers effect. Although it has gained some progress compared to previous works, its clipping strategy is still detrimental to clean images. Besides, the calculation of  IFNR and the introduction of FNC layers with the L-2 norm will also increase the difficulty of this algorithm utilization and the complexity of deep CNNs. Moreover, those approaches mentioned above are difficult to deploy on front-end devices because their detection relies to some extent on the original deep CNNs. Since advanced edge devices (such as which built-in CMOS sensors~\cite{}) allow for lightweight Neural Networks computing, that inspired us to find an efficient and low-cost way to detect adversarial patches with edge devices.  

In contrast to previous methods that require modification of the original models, we proposed the first framework based on edge-device to guarantee the security of deep CNNs applications. As shown in Fig.~\ref{fig:Fig1}, we present a lightweight unified model embedded in edge devices that is efficient in detecting various adversarial patches. In terms of application, our approach is more feasible because we do not need to modify the models in back-end devices or adjust our model according to the changes in the back-end model. % 再加点实验结果，精度，计算量等。

% In summary, the method proposed in this paper has greatly reduced computational and deployment costs for adversarial patches detection and its application field is wide. The experiment shows its F1-score can reach 97\% in the detection of all kinds of adversarial patches.


==> _his/1-Introduction_v3.tex <==
\section{Introduction}
% 以下需要往边缘设备上靠，引出我们的动机
Edge devices and sensors usually run in a complex and noisy environment, where data are exposed to contamination with a high possibility. Combating these contamination usually caused by adversarial attacks in visual intelligent service requires neural networks with specific anti-interference optimization.
However, the extremely limited computing resources of edge devices severely limit the near-sensor deployment of high-workload robustness-strengthened neural networks.
%Although there have been some attempts to compute near-sensor convolutional neural networks, their compression and modification of neural network cause some damages to the models, among which vulnerability to adversarial attack is extraordinarily significant.
As a result, given security concerns in practical applications, the centralised approach is still the most commonly used in industry. 
In this mode, all the data collected by the sensor end will be transmitted to the central computing end regardless of perturbations and even attacks, and robustness-strengthened neural networks on the central computing end will shoulder the responsibility of fighting such adversarial attacks.
This creates redundant communication overhead and increases the workload on the computing center, which goes against the trend towards distributed and near-sensor computing.
%接下来一段的思路是阐述没有必要把被污染的数据传到back-end进行计算，既能减小communication开销，又能减小back-end的计算负载（这个怎么写一段需要想一下）
%接下来一段讲adversarial patches的一些特性（low-level feature， high activation），（说明现有的对抗adversarial patches的方法是怎么在我们的这个场景下失效的），以及adversarial patches的特性启发了near-sensor的AP detection

In recent years, near-sensor computing has made significant progress in its ability to execute lightweight neural network workloads. One promising technology is the neuromorphic system with crossbar structures, which provides efficient implementations of near-sensor computing by simulating the biological brain's synapses, neurons, and kinetics.
%Using Ohm's law and Kirchhoff's law, the neuromorphic system can directly compute the matrix-vector multiplication (MVM) of neural networks in parallel without the need to digitize the outputs of sensors. 
The emergence of advanced edge devices, such as resistive memory (ReRAM) devices~\cite{}, has further facilitated the efficient running of lightweight neural networks in the neuromorphic system. Exploring the potential of deploying a dedicated lightweight neural network at edge devices that utilizes near-sensor computing for real-time detection of visual attacks could prevent contaminated data from being transmitted to the back-end computing center. This novel strategy can effectively reduce redundant communication and computational load on the back-end, while also being a cost-effective solution for preventing visual attacks as it does not require custom defenses optimization for existing back-end neural networks that are already in use.

Adversarial patch attacks~\cite{eykholt2018robust, brown2017adversarial, karmon2018lavan} have emerged as an urgent threat among various adversial attacks~\cite{szegedy2013intriguing,goodfellow2014explaining,kurakin2018adversarial,moosavi2016deepfool,carlini2017adversarial,eykholt2018robust,brown2017adversarial,karmon2018lavan}. In this type of attack, a small yet carefully-crafted patch is placed randomly on an image obtained by the sensor. These patches have been proven to cause the back-end neural networks to generate abnormal activation layer by layer~\cite{yu2021defending}, which weakens the authentic features of the original image and deceives the back-end system into misidentifying the image. The simplicity of training and the low-cost deployment of such attacks makes them attractive to malicious actors seeking vulnerabilities in visual intelligence systems. As a result, the trustworthiness and reliability of these systems are compromised.
%, including but not limited to facial recognition, object detection, autonomous driving, and surveillance systems
Thus, it is imperative to detect adversarial patch attacks.

Many works have proposed solutions to tackle the security issue of back-end intelligence system caused by adversarial patch attacks. However, none of these solutions are currently applicable to edge devices. For instance, Digital Watermarking (DW)~\cite{hayes2018visible} and Local Gradient Smoothing (LGS)~\cite{naseer2019local} have been proposed as patch removal techniques that locate and either erase or mask patches. %However, they perform poorly in patch detection and often compromise significant parts of the clean image. 
LanCe~\cite{xu2020lance} defined Input Semantic Inconsistency for patch detection,
%, but its computation is too complicated and requires the prediction class of the data, limiting its applicability to post-prediction correction. 
while Yu~\cite{yu2021defending} introduced Feature Norm Clipping (FNC) layer between layers of the model and defined the Incremental Feature Norm Ratio (IFNR) to assess the effectiveness of FNC layers.
%, but its clipping strategy still damages clean images. Moreover, calculating IFNR and introducing FNC layers with the L-2 norm increase the algorithm's complexity and the neural network's computational overhead. 
%In summary, 
These approaches cannot be implemented on edge devices as their patch detection or removal depends on specifically optimized neural networks for the original back-end models, which is both time-consuming and resource-intensive. 

In contrast to previous methods that require custom optimization of the back-end neural networks, we propose the first framework that exploits edge devices to develop an effective and cost-efficient method to enhance the security of visual intelligence systems. As shown in Fig.~\ref{fig:Fig1}, our approach employs a universal lightweight neural network embedded in edge devices to detect various types of adversarial patches by identifying abnormal values in the attention map. Our approach offers greater adaptability for applications as it eliminates the need to customize the back-end neural networks or adjust our edge-built model to match the back-end system. By preventing contaminated data from being uploaded, our approach reduces communication bandwidth, enhances the accuracy of the back-end intelligence system, and reduces its workload. Our framework is applicable to a wide range of visual intelligence systems and can help improve the overall security and efficiency of these systems. % 再加点实验结果，精度，计算量等。

% In summary, the method proposed in this paper has greatly reduced computational and deployment costs for adversarial patches detection and its application field is wide. The experiment shows its F1-score can reach 97\% in the detection of all kinds of adversarial patches.

==> _his/1-Introduction_v4.tex <==
\section{Introduction}
% 以下需要往边缘设备上靠，引出我们的动机
Edge devices and sensors usually run in a complex and noisy environment, where data are exposed to contamination with a high possibility. Combating these contamination usually caused by adversarial attacks requires deep neural network (DNN) with specific anti-interference optimization.
However, the extremely limited computing resources of edge devices severely limit local deployment of high-workload robustness-strengthened neural networks.
%Although there have been some attempts to compute near-sensor convolutional neural networks, their compression and modification of neural network cause some damages to the models, among which vulnerability to adversarial attack is extraordinarily significant.
As a result, given security concerns in practical applications, the centralised approach is still the most commonly used. 
In this mainstream mode, all the data collected by the edge sensor end will be transmitted to the central computing end (back end) regardless of perturbations and even attacks, and robustness-strengthened neural networks on the back end will shoulder the responsibility of fighting such adversarial attacks.
This creates redundant communication overhead and increases the workload on the computing center, which goes against the trend towards edge computing.
%接下来一段的思路是阐述没有必要把被污染的数据传到back-end进行计算，既能减小communication开销，又能减小back-end的计算负载（这个怎么写一段需要想一下）
%接下来一段讲adversarial patches的一些特性（low-level feature， high activation），（说明现有的对抗adversarial patches的方法是怎么在我们的这个场景下失效的），以及adversarial patches的特性启发了near-sensor的AP detection

Among various adversarial attacks, adversarial patch attacks -- a small yet carefully crafted patch is placed randomly on an image obtained by the sensor~\cite{eykholt2018robust, brown2017adversarial, karmon2018lavan} have emerged as an urgent threat ~\cite{szegedy2013intriguing,goodfellow2014explaining,kurakin2018adversarial,moosavi2016deepfool,carlini2017adversarial,eykholt2018robust,brown2017adversarial,karmon2018lavan}. These patches have been proven to cause the back-end neural networks to generate abnormal activation layer by layer~\cite{yu2021defending}, which weakens the authentic features of the original image and deceives the back-end system into misidentifying the image. The simplicity of training and the low-cost deployment of such attacks makes them attractive to malicious actors seeking vulnerabilities in visual intelligence systems. As a result, the trustworthiness and reliability of these systems are compromised.
%, including but not limited to facial recognition, object detection, autonomous driving, and surveillance systems
Thus, it is imperative to detect adversarial patch attacks and remove them during the neural networks processing.

In recent years, emerging near (or in)-sensor computing architectures~\cite{du2015shidiannao,likamwa2016redeye, liu20191, ma2019analog} have been proposed to enhance the edge computing efficiency. By moving some executions closer to the sensor nodes, these designs save data movements, storage, and bandwidth. 
Moreover, these architectures are easily integrated with the CMOS image sensor (CIS) module - a component of intelligent visual perception systems - allowing for always-on applications~\cite{ma2019analog}. Coupled with computing-in-memory (CIM) techniques~\cite{chi2016prime, yang201924, liu2020ns}, which conduct computation in analog domain, they effectively accelerate neural network processing on edge devices, making real-time processing possible.
% ShiDianNao hoists the CNN accelerator next to the CMOS or CDD sensor to entirely eliminate the DRAM accesses.
% RedEye pushes early processing of ConvNet into the analog domain that processes near sensors to reduce the workload of the analog readout. 
% Fei Qiao's group designs a visual perception chip that directly attaches the analog processing unit of BNN to CIS. This ADC-free architecture reaches ultra-low power consumption and high energy efficiency.
% In recent years, the substantial advancements in near-sensor computing have enhanced the capacity of edge devices to carry out lightweight neural network workloads. It can be easily integrated with prevalent CMOS image sensor (CIS) modules for always-on application to realize real-time data processing.
% One promising technology is the neuromorphic system with crossbar structures, which provides efficient implementations of near-sensor computing by simulating the biological brain's synapses, neurons, and kinetics.
%Using Ohm's law and Kirchhoff's law, the neuromorphic system can directly compute the matrix-vector multiplication (MVM) of neural networks in parallel without the need to digitize the outputs of sensors. 
% The emergence of advanced edge devices, such as resistive memory (ReRAM) devices~\cite{}, has further facilitated the efficient running of lightweight neural networks in the neuromorphic system. 
Exploring the potential of deploying a dedicated lightweight neural network at edge devices that utilizes near-sensor computing for real-time detection of visual attacks could prevent contaminated data from being transmitted to the back-end computing center. This novel strategy can achieve real-time data cleaning without waiting for the back-end processing and also effectively reduce redundant communication and computation load on the back-end. 

Although many works have been proposed to tackle the security issue of intelligence systems caused by adversarial patch attacks, none of them are feasible to be deploy on edge devices. 
For example, Digital Watermarking (DW)~\cite{hayes2018visible} and Local Gradient Smoothing (LGS)~\cite{naseer2019local} were proposed as patch removal techniques that locate and erase (or mask) patches. %However, they perform poorly in patch detection and often compromise significant parts of the clean image. 
LanCe~\cite{xu2020lance} defined Input Semantic Inconsistency for patch detection.
%, but its computation is too complicated and requires the prediction class of the data, limiting its applicability to post-prediction correction. 
Yu~\cite{yu2021defending} introduced Feature Norm Clipping (FNC) layer between original model layers.
%, but its clipping strategy still damages clean images. Moreover, calculating IFNR and introducing FNC layers with the L-2 norm increase the algorithm's complexity and the neural network's computational overhead. 
%In summary, 
However, these approaches heavily rely on optimizing the original back-end models, which involves complex execution and large-scale deployment of neural network models. Such resource-intensive processes are not practical for edge devices, where computing power and memory capacity are limited.

%However, these patch detection or removal depend on optimizations on the original back-end models, which involve complex executions and large-scale neural network model deployment.

%depends on specific optimizations on the original back-end models, which are large-scale and need time-consuming and resource-intensive executions. 

\begin{figure*}[!t]
  \vspace{-3mm}
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=7in, height=3.5in]{_fig/Fig1.pdf}
  \caption{The framework of our proposed method.}
  \label{fig:Fig1}
  \vspace{-5mm}
  % \Description{}
\end{figure*}

In our work, we propose an edge computing framework that can effectively and efficiently detect abnormal data using adversarial patches and purify sensory data.
As shown in Fig~\ref{fig:Fig1}, the main component of this framework is a lightweight yet versatile detection model.
It can detect adversarial patches generated for various DNN models.
The detection model is composed of only a few layers from the backend DNN models, which allows it to be deployed locally.
Additionally, we have developed an attention-based methodology to achieve accurate detection while introducing only simple computations.
%The detection model is lightweight, making it resource-efficient and well-supported for edge deployment. Combing computing in memory technology can optimize resource utilization and enables real-time attack detection. With this universal detection model, there is no need to enhance and re-deploy the back-end neural networks that are already widely deployed in the industry. 
% The requirement of adjusting edge-built model to match the back-end system is also eliminated. 
By preventing contaminated data from being transmitted to the back-end cloud, our framework also reduces communication bandwidth, enhances the accuracy, and reduces the workload of the back-end intelligence system. 
%This work provides a promising solution to the issue of AI security.

% Our framework is applicable to a wide range of visual intelligence systems and can help improve the overall security and efficiency of these systems. 

% 再加点实验结果，精度，计算量等。
% In summary, the method proposed in this paper has greatly reduced computational and deployment costs for adversarial patches detection and its application field is wide. The experiment shows its F1-score can reach 97\% in the detection of all kinds of adversarial patches.



==> _his/2-Background_v1.tex <==
\newpage
\section{Background}
\subsection{AI Trustworthiness}
% 简要介绍深度神经网络的发展，带出常被攻击的经典CNN模型,即为后文实验用的 thread model
% 介绍adversarial patch, 与传统 adversarial attack 进行区分，以及由于adversarial patch的训练和部署成本低，应用广泛且难以预防，本文关注对adversarial patch 的预防。

\begin{figure*}[t]
  \vspace{-3mm}
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=7in, height=3.5in]{_fig/Fig1.pdf}
  \caption{The framework of our proposed method.}
  \label{fig:Fig1}
  \vspace{-3mm}
  % \Description{}
\end{figure*}

In recent years, with the competition events of image classification tasks held, various deep learning models have developed and reached prominent results, such as VGG-16~\cite{simonyan2014very}, ResNet-50~\cite{he2016deep}, MobileNet-V2~\cite{sandler2018mobilenetv2}, Inception-V3~\cite{szegedy2016rethinking}, ResNet-101~\cite{he2016deep} etc. They are increasingly utilized in wide fields of the physical world. These models are large in scale and complex in structure and are often deployed in the server to classify uploaded images. The CNN units are important components of each layer of models, which can effectively extract location features and high-level semantic features of images. But these models are susceptible to attack. Instead of attacking the neural units of the model, attackers simply perturb a small number of pixels of the inputs can make a huge difference to the model results. For example, classify a fiddler crab as a white shark, as shown in Fig.~\ref{fig:Fig1}.

At first, the perturbed pixels are scattered throughout the whole image and are unnoticeable to the human~\cite{szegedy2013intriguing}. The cost of this kind of adversarial attack is attackers need to train specific perturbations for each image. Subsequently, adversarial patch attack was gradually proposed and implemented more often. When applying the adversarial patch attack, attackers simply need to train a universal patch against the threat model with a small dataset and then attach it to any location of the input images~\cite{brown2017adversarial}.

\subsection{AI Safeguard}
% 1.详细介绍 DW, LGS, LanCe, Yu 的方法
% 2.指出他们方法的不足
% 3.另外，他们的方法都有一个共同的缺陷，他们的方法对clean样本的影响没有进行实验分析，
% 如LanCe中，对detection检测，所有测试样本均为被attack的样本，从而求的检测的acc,并没有分析现实情况中，攻击是未知的，可能模型的input是完全clean,也可能部分input被attack，因此他们的实验结果的评价指标不够客观。
% Lance中使用的patch仅仅是针对Inception-V3训练的，虽然patch有high transferability的属性，但是从后续实验结果来看，其对不同模型的攻击性是有差别的，该论文提出的方法能较好检测出该patch，却不一定能检测出更有针对性训练的patch.
Adversarial patches attacks have raised concerns about the security of deep CNNs, and several methods have been proposed. Digital Watermarking (DW) locates and erases patches~\cite{hayes2018visible}. Local Gradient Smoothing (LGS) applies a soft mask to images during the pre-processing stage of inputs~\cite{xu2020lance}. They reconstructed the attacked image so that the model's accuracy on those images is well recovered, but the clean images are reconstructed as well because of the poor performance of patch detection, which may leads to a decrease in the model's accuracy on these clean images. LanCe defines an inconsistency between the output of the model's last layer and the synthesized pattern of its predicted category. When the inconsistency is greater than a threshold, they consider the input to be attacked~\cite{xu2020lance}. If the number of classification categories is hundreds, it means that there will be hundreds of synthesized patterns and associated thresholds that need to be computed as the preparation of inconsistency calculation. Yu proposed adding FNC layers to clip the outputs of several specific layers of the model. They defined the IFNR metric as well to demonstrate that the effect of patches on IFNR values is suppressed after outputs of selected layers are processed by FNC layers. The clipping strategy of FNC is to replace  the values of all points in the feature map where L-2 norm are greater than the mean~\cite{yu2021defending}. Since the larger values of the feature map contribute more to the classification result, this clipping strategy obviously has an impact on the classification of clean images. In addition, the IFNR computation and NFC layers increase the complexity of the original model.


==> _his/2-Background_v2.tex <==
% \newpage
\begin{figure*}[t]
  \vspace{-3mm}
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=7in, height=3.5in]{_fig/Fig1.pdf}
  \caption{The framework of our proposed method.}
  \label{fig:Fig1}
  \vspace{-3mm}
  % \Description{}
\end{figure*}

\section{Background}
\subsection{AI Trustworthiness}
% 简要介绍深度神经网络的发展，带出常被攻击的经典CNN模型,即为后文实验用的 thread model
% 介绍adversarial patch, 与传统 adversarial attack 进行区分，以及由于adversarial patch的训练和部署成本低，应用广泛且难以预防，本文关注对adversarial patch 的预防。
The increasing advancements in deep convolutional neural networks (CNNs) have led to their widespread adoption in various visual intelligence systems, including but not limited to facial recognition, object detection, autonomous driving, and surveillance systems. Typical and powerful CNNs, such as VGG-16~\cite{simonyan2014very}, ResNet-50~\cite{he2016deep}, MobileNet-V2~\cite{sandler2018mobilenetv2}, Inception-V3~\cite{szegedy2016rethinking}, and ResNet-101~\cite{he2016deep} have large scales and complex structures. However, these models are vulnerable to visual attacks, particularly adversarial patch attacks, where a small universal patch trained on a limited dataset is attached to the model's inputs~\cite{brown2017adversarial}. Patches trained against one model exhibit varying levels of transferability to other models. Thus, this paper focuses on developing a universal and efficient method for detecting all adversarial patches trained against varying models. 

Although many approaches have been proposed to address this issue, they all suffer from certain limitations. DW~\cite{hayes2018visible} and LGS~\cite{xu2020lance} perform poorly in patch detection and can compromise significant parts of the clean image. LanCe~\cite{xu2020lance} detects inconsistencies between the output of the model's last layer and the synthesized pattern of the predicted category. However, this approach requires computing thresholds for synthesized patterns of each category, which can be time-consuming. Furthermore, the computation of the inconsistency requires knowledge of the predicted class of the output, limiting its use to post-prediction correction.
Yu et al.~\cite{yu2021defending} proposed adding FNC layers to clip the outputs of specific layers in the model. They also defined the IFNR metric to demonstrate that the impact of patches on IFNR values is mitigated after processing the outputs of selected layers with FNC layers. The FNC clipping strategy involves replacing the values of all points in the feature map where the L-2 norm is greater than the mean. However, this clipping strategy also affects the larger values in the feature map of clean images that contribute more to the classifier's output, resulting in noticeable damage to the clean images. Moreover, the computation of IFNR and the introduction of FNC layers increase the algorithm's complexity and the neural network's computational overhead.

%To analyze the impact of adversarial patches on these models, we trained patches against each model with 2000 images from ImageNet and then evaluate the top-1 accuracy of each model under path attacks, as presented in Table 1. It showed that adversarial patch have varying degrees of transferability. VGG-16 and Inception-V3 are more susceptible to patch attacks, while MoblieNet-V2 is relatively robust. This provides a possible explanation for the higher transferability of the patch trained against MobileNet-V2 (AdvP-MobileNetV2) and its relative difficulty to detect, as demonstrated in subsequent experiments (table 2 and table 3).

\subsection{Near-Sensor Computing}
% 介绍部分工作是怎么做的，以及ReRAM用于neuromorphic computing
% 说明将检测移到edge端的必要性
The emergency technology of near-sensor computing provides a novel avenue to tackle the issue of AI trustworthiness. Near-sensor computing is a rapidly evolving field within edge computing that seeks to bring computation closer to the data source by embedding processing capabilities directly into sensor nodes. This paradigm dramatically reduces data movement, cutting down on energy consumption and latency, thus making real-time visual attacks detection feasible.

To boost the computing efficiency of near-sensor processing, emerging technologies like ReRAM are incorporated for neuromorphic computing. ReRAM is a type of non-volatile memory that leverages material resistance to store data, offering high endurance and low power consumption. When used for neuromorphic computing, it can effectively emulate the structure and functionality of neural networks, thereby offering a natural fit for AI computations on edge devices.

Moving visual attack detection to the edge via near-sensor computing is significant. First, it reduces latency and energy consumption, as the need to transfer raw data to the cloud for processing is eliminated. Second, on-device detection enhances security as it prevent data may include Trojan attacks from uploading. As such, leveraging near-sensor computing with ReRAM for neuromorphic computing in visual attack detection presents a practical, efficient, and robust approach for improving the security of real-world AI applications.





==> _his/2-Background_v3.tex <==
\section{Background}
\subsection{AI Robustness}
% 简要介绍深度神经网络的发展，带出常被攻击的经典CNN模型,即为后文实验用的 thread model
% 介绍adversarial patch, 与传统 adversarial attack 进行区分，以及由于adversarial patch的训练和部署成本低，应用广泛且难以预防，本文关注对adversarial patch 的预防。
The increasing advancements in DNNs have led to their widespread adoption in various AI systems, including but not limited to facial recognition, object detection, autonomous driving, and surveillance systems. The large-scale DNNs such as VGG-16~\cite{simonyan2014very}, ResNet-101~\cite{he2016deep}, MobileNet-V2~\cite{sandler2018mobilenetv2}, etc. %Inception-V3~\cite{szegedy2016rethinking}, and ResNet-101~\cite{he2016deep} 
are powerful with complex structures. 
However, these models are vulnerable to visual attacks, particularly adversarial patch attacks, where a small universal patch trained on a limited dataset is attached to the model's inputs~\cite{brown2017adversarial}. Patches trained against one model exhibit varying levels of transferability to other models. Therefore, this work focuses on developing a universal and light-weight model with low-cost detection methodology for detecting all adversarial patches trained against varying models. 

Although many approaches have been proposed to address this issue, they all suffer from certain limitations. DW~\cite{hayes2018visible} and LGS~\cite{naseer2019local} perform poorly in patch detection and can
compromise significant parts of the clean image. LanCe~\cite{xu2020lance} detects inconsistencies between the output of the model's last layer and the synthesized pattern of the predicted category. 
This approach requires computing thresholds for synthesized patterns of each category, which is resource- and time-consuming. 
Furthermore, the computation of the inconsistency requires knowledge of the predicted class of the output, limiting its use to post-prediction correction.
Yu et al.~\cite{yu2021defending} proposed adding FNC layers to clip the outputs of specific layers in the model. 
%They also defined the IFNR metric to demonstrate that the impact of patches on IFNR values is mitigated after processing the outputs of selected layers with FNC layers. 
The FNC clipping strategy involves replacing the values of all points in the feature map where the L-2 norm is greater than the mean. 
However, this clipping strategy also affects the larger values in the feature map of clean images that contribute more to the classifier's output, resulting in noticeable damage to the clean images. 
Moreover, the introduction of FNC layers increase the algorithm complexity and the involved computations are resource expensive.
It is noted that these methods involve full neural network models, which also hinders their deployment on edge devices.

%To analyze the impact of adversarial patches on these models, we trained patches against each model with 2000 images from ImageNet and then evaluate the top-1 accuracy of each model under path attacks, as presented in Table 1. It showed that adversarial patch have varying degrees of transferability. VGG-16 and Inception-V3 are more susceptible to patch attacks, while MoblieNet-V2 is relatively robust. This provides a possible explanation for the higher transferability of the patch trained against MobileNet-V2 (AdvP-MobileNetV2) and its relative difficulty to detect, as demonstrated in subsequent experiments (table 2 and table 3).

\subsection{Near-Sensor Computing}
% 介绍部分工作是怎么做的，以及ReRAM用于neuromorphic computing
% 说明将检测移到edge端的必要性

Near-sensor computing is a rapidly evolving field within edge computing that seeks to bring computation closer to the data source by embedding processing capabilities near sensor sides. 
The emerging of near-sensor computing provide a novel avenue to tackle the issue of AI robustness. 
% This paradigm dramatically reduces data movement, cutting down on energy consumption and latency, thus making real-time visual attacks detection feasible.

ShiDianNao~\cite{du2015shidiannao} hoists the DNN accelerator next to the CMOS sensor to eliminate the DRAM accesses.
RedEye~\cite{likamwa2016redeye} pushes early processing of ConvNet into the analog domain that processes near sensors to reduce the workload of the analog readout.
Qiao's group designs a visual perception chip that directly attaches the analog processing unit of binary nerual network to CIS, which eliminates the large analog circuits (e.g., ADC) needs and achieves high energy efficiency~\cite{liu20191}. 
%This architecture design eliminates the need for ADC and conventional analog buffers, reaching ultra-low power consumption and high energy efficiency. 
% This ADC-free architecture reaches ultra-low power consumption and high energy efficiency.
They also propose an analog-memoryless near-sensor computing architecture that shifts the correlating-double-sampling (CDS) operation to the Computation Module to reduce hardware overhead~\cite{ma2019analog}. %This move leads to a reduction in hardware overhead and an enhancement in energy efficiency.
NS-CIM~\cite{liu2020ns} integrates near-sensor computing architecture with CIM paradigm to process sensory signals locally, significantly cutting down on data conversion and movement.

\begin{figure}[t]
  \vspace{-3mm}
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.0cm}
  \centering
  \includegraphics[width=\linewidth]{_fig/Fig2.pdf}
  \caption{Attention values of clear and perturbed data.}
  \label{fig:Fig2}
  \vspace{-4mm}
  % \Description{}
\end{figure}

\begin{figure*}[t]
  \vspace{-3mm}
  \setlength{\abovecaptionskip}{1.3mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=\textwidth,height=1.4in]{_fig/Fig3.pdf}
  \caption{Distributions of $I_{r}$ indicators at different layers of VGG-16 on ImageNet.}
  \label{fig:Fig3}
  \vspace{-3mm}
  % \Description{}
\end{figure*}

By leveraging near-sensor computing and CIM, our developed adversarial data detection can be easily deployed to the edge, enabling real-time data purification and robust AI systems.
%1) reduce latency and energy consumption as the need to transfer raw data to the cloud for processing is eliminated, 2) enhance AI system roubustness as it prevent data may include Trojan attacks from uploading. As such, leveraging near-sensor computing with CIM technology in visual attack detection presents a practical, efficient, and robust approach for improving the security of real-world AI applications.





==> _his/3-Method_v1.tex <==
\section{Proposed Adversarial Patches Detection}
% 1. 附上部署的框架图（类似EARLIN的整合图3：collaborative inference）以及detection 部分的框架图(类似EARLIN的图1)，介绍模型包含哪几部分(detection、classify)

In this section, we will introduce our method for early adversarial patch detection on edge devices. As shown in Fig.~\ref{fig:Fig1}, the framework of our work consists of two parts: detection and inference. The detection is deployed on an edge device that collects inputs through sensors. That stage will make use of the shallower layers output of VGG-16. After detection, only if the input is detected as a clean image will it be uploaded to the server for inference. The inference part is a full deep CNN deployed on the server, proven excellent in classification, such as VGG-16, ResNet-101, Inception-V3, etc. Note that we only upload the original image instead of the intermediate output of VGG-16 to reduce the bandwidth pressure during the upload.

\begin{figure}[t]
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.0cm}
  \centering
  \includegraphics[width=\linewidth]{_fig/Fig2}
  \caption{Samples perturbed by adversarial patch at different locations.}
  \label{fig:Fig2}
  \vspace{-5mm}
  % \Description{}
\end{figure}

\subsection{Analysis of Adversarial Patches Attacks}
% 1. 介绍attention map ,公式和意义，并与传统的 attention 机制（attention 因子是模型在训练过程中需要进行学习的参数）进行区分
% 2. 并附上被adversital patch 攻击后的对比图，包括attention map热力图和柱状分布图(最后一层conv)
% 3. 分析patch位置对attention map的影响，附上在图片边缘部位attack后的热力图
It is observed that adversarial patches mislead classifier result by causing some signiﬁcant abnormalities that overwhelm the original decision portion in the last convolution activation map~\cite{xu2020lance,yu2021defending}. Instead of introducing complex calculations of L-2 norm or similarity, we will leverage attention mechanism~\cite{yu2022antidotex} to analyze the change of activation map at different layers. We can calculate every point's value in attention map as Eq. 1.
\begin{equation}
A_{T}(F,h,w) = \frac{1}{C} \sum_{i}^{C}F_{h,w}(i)
\end{equation}
$F\in \mathbb{R}^{C\ast H\ast W}$ is the activation map for a layer of the model. $F_{h,w}(i)$ represent the activation value of $i^{th}$ channel at coordinates \begin{math} (h,w)\end{math} of activation map. The attention map calculates activation map's mean in the dimension of channel depth C. So, we would get a attention map $A_{T}(F)$ of $H\ast C$ size for $F$.

\begin{figure*}[b]
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=0.8\textwidth]{_fig/Fig3}
  \caption{An example of attention maps at different layers of VGG-16.}
  \label{fig:Fig3}
  \vspace{-3mm}
  % \Description{}
\end{figure*}

We used the original adversarial patch method~\cite{brown2017adversarial} to train an adversarial patch against VGG-16~\cite{simonyan2014very} with small part samples (2000) from Imagenet~\cite{russakovsky2015imagenet}. This patch with a size of only 6\% of the original image dropped the top-1 accuracy of VGG-16 to 1.3\% on Imagenet. At first, we observed its influence on the attention map at the last convolution layer. Fig.~\ref{fig:Fig2} shows two examples that the original image and perturbed will get into huge differences at the place of the patch, where the perturbed will be significantly higher in values. We further selected different layers to analyze the influence of adversarial patch attacks. Fig.~\ref{fig:Fig3} tells that the difference shows up earlier than we thought. That inspired us to take advantage of this early difference for detection. So we are supposed to define an indicator to represent the whole attention map that will better maximize the difference. As shown in Fig.~\ref{fig:Fig3}, the values range of a attention map is relatively narrow before the attack. But the patch considerably increased the upper limit of the range at all layers. So we will take the upper limit of range as the indicator for one attention map, which defined by:

We generated $I_{r}$ indicators with 20,000 perturbed images and their corresponding clean images from Imagenet~\cite{russakovsky2015imagenet}. For different layers of VGG-16, the frequency histograms of $I_{r}$ are shown in Fig.~\ref{fig:Fig4}. It suggested that the earlier the layer is, the greater the separation between clean and perturbed $I_{r}$ distributions. Intuitively, $I_{r}$ is a perfect indicator for us to early detect adversarial patch. 


To support our assumption, we also defined another indicator $I_{c}$ by calculating the average of attention map in the dimension $H\ast W$:
\begin{equation}
I_{c}(F) = \frac{1}{H\ast W}\sum_{h}^{H}\sum_{w}^{W}A_{T}(F,h,w)
\end{equation}
The frequency histograms of $I_{c}$ are shown in Fig.~\ref{fig:Fig6}. It shows an opposite trend to $I_{r}$: the earlier the layer is, the higher the overlap between the distributions of clean and perturbed $I_{c}$. The different trends shown in Fig.~\ref{fig:Fig4} and Fig.\ref{fig:Fig5} may be interpreted with the principle of the convolution operation. At the early layer, the patch impact that increases values in the attention map is concentrated at the patch location. As the patch size is only 6\% of the original image, its influence on $I_{c}$ will be reduced by the average operation. However, as the layers go deeper, the patch impact will be carried to more places through the cascade convolution operation. But the degree of impact at each point is diminishing. That will raise its influence on $I_{c}$ but drop on $I_{r}$.

Even in the last layer, the distributions of $I_{c}$ still overlap, while the distributions of $I_{r}$ remain separate, making $I_{r}$ a more suitable indicator for detection than $I_{c}$, especially at the early layer.  

\subsection{Adversarial Patches Detection}
% 1. 介绍detection 的方法，如何求 Threshold 值并用于检测的公式。
% 附上vgg16模型的图，标记我们取的进行attent map 分析的各层
% 附上各层layer的Max(attent map)分布的频率图
% 2. 用各层频率分离图说明浅层用于检测的合理性
% 1）浅层相比最后一层分离更明显，并对这个现象给出自洽的解释
% 2）利用浅层进行检测能在更早期时候检测patch,节省计算资源，更有利于部署
In this section, we will describe how to use $I_{r}$ for detection. Since the distributions of clean and perturbed $I_{r}$ are separate, we can easily find a threshold value, $\Theta$, with only $I_{r}$ of clean samples. Using the threshold we can detects clean samples with some confidence $p$ at early layer. 
\begin{equation}
p = \frac{\sum_{F\in F_{clean}}\mathbb I(I_{r}(F)\leq \Theta)}{|F_{clean}|}
\end{equation}
$F_{clean}$ represents a list of activation maps generated from plenty of clean samples. $|F_{clean}|$ indicates the number of elements in $F_{clean}$. The symbol $\mathbb I()$ is the indicator function that returns $1$ if the condition in parentheses is True, $0$ otherwise. Given a value of $p$, we calculate a threshold $\Theta$ indicating that $p$ fractions of the clean samples satisfy $I_{r}(F)\leq \Theta$. As shown the red vertical line in Fig. 5, we empirically set $p=0.95$. This is actually the expected capability of our patch detector to detect a true clean sample as clean. It is important to note that our method of calculating the value of $\Theta$ does not require exposure to any perturbed samples.



Finally, the detection of adversarial patches can be formulated as Eq. 5.
\begin{equation}
\mathcal{D}(x) = 
\begin{cases}
1, \quad {if} \ \ {I_{r}(F)>\Theta},\\
0, \quad {otherwise.}
\end{cases}
\end{equation}
For an input sample $x$, we get its activation map $F$ on a selected early convolution layer of VGG-16. Then we calculate its $I_{r}$ indicator through Eq. 1 and Eq. 2. The cascaded model from the first to the selected layer of VGG-16 is our detection model. Perturbed images are taken as positive samples and clean ones as negative samples. We note that all models (VGG-16, ResNet-101, Inception-V3, etc.) used in this paper do not require any training——their weights are fed using pre-trained models of the official. 



Next section, we will introduce our experiments and analyze the results. The experiments will explore the early layers of which model is suitable as a unified model for various adversarial patches detection and how to determine the selected layer.

\begin{figure*}[t]
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=6.6in,height=2in]{_fig/Fig4}
  \caption{Distributions of $I_{r}$ indicators at different layers of VGG-16 on ImageNet.}
  \label{fig:Fig4}
  \vspace{-3mm}
  % \Description{}
\end{figure*}

\begin{figure*}[t]
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=0.9\textwidth,height=7.5cm]{_fig/Fig5}
  \caption{Distributions of $I_{r}$ indicators at different layers of VGG-16 on ImageNet.}
  \label{fig:Fig5}
  \vspace{-3mm}
  % \Description{}
\end{figure*}

% \begin{figure*}[b]
%   \setlength{\abovecaptionskip}{1.4mm}
%   \setlength{\belowcaptionskip}{-0.cm}
%   \centering
%   \includegraphics[width=0.9\textwidth,height=7cm]{_fig/Fig7}
%   \caption{The Process of calculating threshold and of experiments for model evaluation.}
%   \label{fig:Fig7}
%   \vspace{-3mm}
%   % \Description{}
% \end{figure*}

==> _his/3-Method_v2.tex <==
\section{Proposed Adversarial Patches Detection}
% 1. 附上部署的框架图（类似EARLIN的整合图3：collaborative inference）以及detection 部分的框架图(类似EARLIN的图1)，介绍模型包含哪几部分(detection、classify)

In this section, we will introduce our method for early adversarial patch detection on edge devices. As shown in Fig.~\ref{fig:Fig1}, the framework of our work consists of two parts: detection and inference. The detection is deployed on an edge device that collects inputs through sensors. That stage will make use of the shallower layers output of VGG-16. After detection, only if the input is detected as a clean image will it be uploaded to the server for inference. The inference part is a full deep CNN deployed on the server, proven excellent in classification, such as VGG-16, ResNet-101, Inception-V3, etc. Note that we only upload the original image instead of the intermediate output of VGG-16 to reduce the bandwidth pressure during the upload.

\begin{figure}[t]
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.0cm}
  \centering
  \includegraphics[width=\linewidth]{_fig/Fig2.pdf}
  \caption{Samples perturbed by adversarial patch at different locations.}
  \label{fig:Fig2}
  \vspace{-5mm}
  % \Description{}
\end{figure}

\subsection{Analysis of Adversarial Patches Attacks}
% 1. 介绍attention map ,公式和意义，并与传统的 attention 机制（attention 因子是模型在训练过程中需要进行学习的参数）进行区分
% 2. 并附上被adversital patch 攻击后的对比图，包括attention map热力图和柱状分布图(最后一层conv)
% 3. 分析patch位置对attention map的影响，附上在图片边缘部位attack后的热力图
It is observed that adversarial patches mislead classifier result by causing some signiﬁcant abnormalities that overwhelm the original decision portion in the last convolution activation map~\cite{xu2020lance,yu2021defending}. Instead of introducing complex calculations of L-2 norm or similarity, we will leverage attention mechanism~\cite{yu2022antidotex} to analyze the change of activation map at different layers. We can calculate every point's value in attention map as Eq. 1.
\begin{equation}
A_{T}(F,h,w) = \frac{1}{C} \sum_{i}^{C}F_{h,w}(i)
\end{equation}
$F\in \mathbb{R}^{C\ast H\ast W}$ is the activation map for a layer of the model. $F_{h,w}(i)$ represent the activation value of $i^{th}$ channel at coordinates \begin{math} (h,w)\end{math} of activation map. The attention map calculates activation map's mean in the dimension of channel depth C. So, we would get a attention map $A_{T}(F)$ of $H\ast C$ size for $F$.

\begin{figure*}[t]
  \vspace{-3mm}
  \setlength{\abovecaptionskip}{1.3mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=\textwidth,height=1.4in]{_fig/Fig3.pdf}
  \caption{Distributions of $I_{r}$ indicators at different layers of VGG-16 on ImageNet.}
  \label{fig:Fig3}
  \vspace{-3mm}
  % \Description{}
\end{figure*}

\begin{figure*}[!b]
  \vspace{3mm}
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=\textwidth,height=1.4in]{_fig/Fig4.pdf}
  \caption{Distributions of $I_{c}$ indicators at different layers of VGG-16 on ImageNet.}
  \label{fig:Fig4}
  \vspace{-3mm}
  % \Description{}
\end{figure*}


We used the original adversarial patch method~\cite{brown2017adversarial} to train an adversarial patch against VGG-16~\cite{simonyan2014very} with small part samples (2000) from Imagenet~\cite{russakovsky2015imagenet}. This patch with a size of only 6\% of the original image dropped the top-1 accuracy of VGG-16 to 1.3\% on Imagenet. At first, we observed its influence on the attention map at the last convolution layer. Fig.~\ref{fig:Fig2} shows two examples that the original image and perturbed will get into huge differences at the place of the patch, where the perturbed will be significantly higher in values. We further selected different layers to analyze the influence of adversarial patch attacks. We found that the difference shows up earlier than we thought. That inspired us to take advantage of this early difference for detection. So we are supposed to define an indicator to represent the whole attention map that will better maximize the difference. As shown in Fig.~\ref{fig:Fig2}, the values range of a attention map is relatively narrow before the attack. But the patch considerably increased the upper limit of the range at all layers. So we will take the upper limit of range as the indicator for one attention map, which defined by:

\begin{equation}
I_{r}(F) = \max A_{T}(F,h,w)
\end{equation}

We generated $I_{r}$ indicators with 20,000 perturbed images and their corresponding clean images from Imagenet~\cite{russakovsky2015imagenet}. For different layers of VGG-16, the frequency histograms of $I_{r}$ are shown in Fig.~\ref{fig:Fig3}. It suggested that the earlier the layer is, the greater the separation between clean and perturbed $I_{r}$ distributions. Intuitively, $I_{r}$ is a perfect indicator for us to early detect adversarial patch. 


To support our assumption, we also defined another indicator $I_{c}$ by calculating the average of attention map in the dimension $H\ast W$:
\begin{equation}
I_{c}(F) = \frac{1}{H\ast W}\sum_{h}^{H}\sum_{w}^{W}A_{T}(F,h,w)
\end{equation}
The frequency histograms of $I_{c}$ are shown in Fig.~\ref{fig:Fig4}. It shows an opposite trend to $I_{r}$: the earlier the layer is, the higher the overlap between the distributions of clean and perturbed $I_{c}$. The different trends shown in Fig.~\ref{fig:Fig3} and Fig.\ref{fig:Fig4} may be interpreted with the principle of the convolution operation. At the early layer, the patch impact that increases values in the attention map is concentrated at the patch location. As the patch size is only 6\% of the original image, its influence on $I_{c}$ will be reduced by the average operation. However, as the layers go deeper, the patch impact will be carried to more places through the cascade convolution operation. But the degree of impact at each point is diminishing. That will raise its influence on $I_{c}$ but drop on $I_{r}$.

Even in the last layer, the distributions of $I_{c}$ still overlap, while the distributions of $I_{r}$ remain separate, making $I_{r}$ a more suitable indicator for detection than $I_{c}$, especially at the early layer.  



\subsection{Adversarial Patches Detection}
% 1. 介绍detection 的方法，如何求 Threshold 值并用于检测的公式。
% 附上vgg16模型的图，标记我们取的进行attent map 分析的各层
% 附上各层layer的Max(attent map)分布的频率图
% 2. 用各层频率分离图说明浅层用于检测的合理性
% 1）浅层相比最后一层分离更明显，并对这个现象给出自洽的解释
% 2）利用浅层进行检测能在更早期时候检测patch,节省计算资源，更有利于部署
In this section, we will describe how to use $I_{r}$ for detection. Since the distributions of clean and perturbed $I_{r}$ are separate, we can easily find a threshold value, $\Theta$, with only $I_{r}$ of clean samples. Using the threshold we can detects clean samples with some confidence $p$ at early layer. 
\begin{equation}
p = \frac{\sum_{F\in F_{clean}}\mathbb I(I_{r}(F)\leq \Theta)}{|F_{clean}|}
\end{equation}
$F_{clean}$ represents a list of activation maps generated from plenty of clean samples. $|F_{clean}|$ indicates the number of elements in $F_{clean}$. The symbol $\mathbb I()$ is the indicator function that returns $1$ if the condition in parentheses is True, $0$ otherwise. Given a value of $p$, we calculate a threshold $\Theta$ indicating that $p$ fractions of the clean samples satisfy $I_{r}(F)\leq \Theta$. As shown the red vertical line in Fig. 5, we empirically set $p=0.95$. This is actually the expected capability of our patch detector to detect a true clean sample as clean. It is important to note that our method of calculating the value of $\Theta$ does not require exposure to any perturbed samples.



Finally, the detection of adversarial patches can be formulated as Eq. 5.
\begin{equation}
\mathcal{D}(x) = 
\begin{cases}
1, \quad {if} \ \ {I_{r}(F)>\Theta},\\
0, \quad {otherwise.}
\end{cases}
\end{equation}
For an input sample $x$, we get its activation map $F$ on a selected early convolution layer of VGG-16. Then we calculate its $I_{r}$ indicator through Eq. 1 and Eq. 2. The cascaded model from the first to the selected layer of VGG-16 is our detection model. Perturbed images are taken as positive samples and clean ones as negative samples. We note that all models (VGG-16, ResNet-101, Inception-V3, etc.) used in this paper do not require any training——their weights are fed using pre-trained models of the official. 

Next section, we will introduce our experiments and analyze the results. The experiments will explore the early layers of which model is suitable as a unified model for various adversarial patches detection and how to determine the selected layer.



==> _his/4-Experiment_v1.tex <==
\section{Experiment and Evaluation}
\subsection{Evaluation Metric and Experiment Process}
% 介绍模型的评价指标P,R,F
% 总的实验框架图，分为分析和测试两步Fig. 7.
\begin{figure*}[t]
  \setlength{\abovecaptionskip}{1.4mm}
  \setlength{\belowcaptionskip}{-0.cm}
  \centering
  \includegraphics[width=0.85\textwidth,height=2.5in]{_fig/Fig5.pdf}
  \caption{The Process of calculating threshold and of experiments for detector evaluation.}
  \label{fig:Fig5}
  \vspace{-5mm}
  % \Description{}
\end{figure*}

Previous work only uses accuracy to evaluate their detection model performance, and their input data are all been attacked. There is a flaw in verifying that their method does not mistake clean images as attacked ones and avoid processing them. Our work attacks half inputs to get positive samples and takes the rest original as negative samples. Besides, our detection model is evaluated with Precision ($P$), Recall ($R$), and F-Score ($F$) metrics, which are known for their objectivity.
% $P$ indicates what percentage of positive prediction samples are truly positive samples. $R$ represents what percentage of positive samples are correctly predicted. $F$ is the weighted harmonic mean of $P$ and $R$, which usually represents the comprehensive performance of the model.
The details of our experiments are shown in Fig.~\ref{fig:Fig5}. First, we perform a stratified random sampling of the dataset ImageNet~\cite{russakovsky2015imagenet} by 4:3:3 to obtain the analysis dataset (40\%) and the test dataset (60\%), respectively. Second, We use original images of the analysis dataset to calculate the threshold $\Theta$ of $I_{r}$ indicators. This threshold is prepared for the subsequent detection of the test dataset. Third, we attack half of the test dataset, thus generating a dataset with balanced positive and negative samples. They are detected by comparing their $I_{r}$ indicators with $\Theta$. Finally, we use the $P$, $R$, and $F$ metrics to evaluate the results of our detection model. In the experiment, our method of calculating the value of threshold does not require exposure to any perturbed samples. The early layers to get $I_{r}$ indicators can also come from other classic models, like ResNet-50, MobileNet-V3, etc. We will discuss the selection of detector models and layers in the Ablation Studies part.

\subsection{Effectiveness of Detection} % Performance of Detection
% 简单介绍针对各种thread models 在Imagenet数据集训练的patch
% vgg16模型的浅层用于检测各种patch，列出实验结果和图，以及模型求出的参数：threshold值
% 实验结果可以和Lance中detection部分进行比较
% 说明在模型应对针对不同网络的patch时，检测层无需做出变更，甚至threshold值都不需要改变
%gpu cost
\input{_tab/tab1}

To start our experiments, we need to train adversarial patches. Although the adversarial patch generated against one model has some transferability, our experiment proves that transferability is limited. As shown in Table~\ref{tab:table1}, we trained adversarial patches against pre-trained classic classifier models with 2000 randomly selected images from ImageNet, respectively. Those patches caused varying degrees of Top-1 accuracy degradation in classical models, especially caused high declines in the networks that trained them. From Table~\ref{tab:table1} we note that the VGG-16 and Inception-V3 are more vulnerable to patches attack, while MoblieNet-V2 is relatively difficult to be attacked. This may result in a more aggressive patch trained on MoblieNet, as shown in Table~\ref{tab:table1}. We aim to build a unified model to detects them all. First, we take early layers of VGG16 as a unified model to get $I_{r}$ indicators and $\Theta$. The detection results for are presented in Table~\ref{tab:table2}. It shows that the best choice for the detector is in the second Conv layer. All attacked inputs (R= 100\%) can be detected correctly and guaranteed at least 95\% of clean images are not taken as attacked. When the edge device is insufficient to deploy the first two Conv layers of VGG-16, the first layer can also be an option.

Next, we performed experiments to further tested the effectiveness of patch detection with shallow layers of other models, as shown in Table~\ref{tab:table3}.

\input{_tab/tab2}

\input{_tab/tab3}

\subsection{Memory and Operation Complexity}
% 将以上各种patch，换其他模型的浅层进行检测, 列出实验结果和图，以及不同的threshold值
% 确定哪个模型的浅层更适合作为统一的检测模型
% 这个确定的过程中，不应该只看实验结果，在实验结果差不多的情况下，应选择浅层结构更简单的模型
% 选择的指导建议
% 浅层结构的复杂度评估：
% 1.计算单元的数量 
% 2.计算过程中需要store并transfer的中间结果数量 
% 3.MADD,FLOPS
% 1.可以找到模型
% 2.实验指导意义



In order to guide the layer and model selection for patch detection, we analyzed the information of each model shallow layer, as shown in Table~\ref{tab:table4}.

\input{_tab/tab4}


\subsection{Reconfigurability Analysis}
% \subsubsection{Patch Detection Applied in Different Fields}
% 针对各种thread models 在 CIFAR-10, CIFAR-100数据集训练patch
% 将以上 patch 用于上一步实验中选出的unified model, 列出实验结果和图，以及不同的threshold值
% 说明当模型应用的领域发生变化时，仅仅需要切换提前计算好的threshold值



==> _his/4-Experiment_v2.tex <==
\section{Experiment and Evaluation}
The experiment details are presented in Fig.~\ref{fig:Fig5}. We perform a 4:6 stratified random sampling of the ImageNet dataset~\cite{russakovsky2015imagenet} to obtain the analysis dataset (40\%) and the test dataset (60\%). Half of the test dataset is randomly attacked to generate a balanced dataset of positive (attacked images) and negative (clean images) samples. Using the analysis dataset, we calculate the threshold $\Theta$ of $I_{r}$ indicators, which we utilized to detect the test dataset.

\subsection{Experiment Setup}
% 介绍模型的评价指标P,R,F
% 总的实验框架图，分为分析和测试两步Fig. 7.

\textbf{Evaluation Metric:} 
Unlike previous research, which evaluated detection models solely based on accuracy using only attacked images as input data, our approach is comprehensively evaluated using commonly used classifier metrics, including precision ($P$), recall ($R$), and F-score ($F$). These metrics require the model's input dataset to consist of both positive and negative samples, allowing us to account for the possibility of falsely classifying clean images as attacked.

\textbf{Detection Layer:} The shallow layers used to obtain $I_{r}$ indicators are taken from VGG-16, but other classic models such as ResNet-50, MobileNet-V3, and others can also be used. The selection of detector models and layers will be discussed in the Ablation Studies section.

\textbf{Attacks Training:} We utilized the original adversarial patch attacks developed by Brown et al.~\cite{brown2017adversarial} to train diverse adversarial patches, which occupy only 6\% of the original image size, against several typical deep CNNs, respectively. We extracted a small sample of 2000 images from Imagenet to train these patches. As presented in Table~\ref{tab:table1}, the top-1 accuracy of the corresponding threat models was reduced to the range of 0.83\% to 33.98\% on Imagenet.

\input{_tab/tab1_v2}

\subsection{Effectiveness of Detection} % Performance of Detection
% 简单介绍针对各种thread models 在Imagenet数据集训练的patch
% vgg16模型的浅层用于检测各种patch，列出实验结果和图，以及模型求出的参数：threshold值
% 实验结果可以和Lance中detection部分进行比较
% 说明在模型应对针对不同网络的patch时，检测层无需做出变更，甚至threshold值都不需要改变
%gpu cost 
From Table~\ref{tab:table1} we observe that adversarial patches cause varying degrees of Top-1 accuracy degradation in classical models, with VGG-16 being the most vulnerable to patch attacks, while MoblieNet-V2 is relatively robust and difficult to attack. We aim to build a unified model to detect all threat models' adversarial patches. 

\input{_tab/tab2}

To accomplish this, we leverage the shallow layers of VGG16 as a unified model to derive the $I_{r}$ indicator and calculate $\Theta$. The detection results, as shown in Table~\ref{tab:table2}, reveal that the second convolutional layer of VGG-16 emerges as the optimal choice for the detection layer, i.e., utilizing the $I_{r}$ indicator, derived from the feature map after the first two layers, offers the best performance in attack detection. All attacked inputs can be correctly identified (R=100\%), and about 95\% of clean images are guaranteed not to be falsely identified as attacked (P$\approx$95\%), with an F-score of at least 97.42\%. The results also suggest that one of the adversarial patches, called Advp-MobileNetV2, which is trained on the robust MobileNet-V2, tends to be more aggressive and exhibits higher cross-model transferability, making it challenging to detect. In scenarios where the edge device is grappling with extreme resource constraints, deploying only the first layer of VGG-16 could still be a viable option. It retains an F-score of at least 87.91\%, even when subjected to the Advp-MoblieNetV2 attack.

% \input{_tab/tab2}

\textbf{Ablation Studies:} We conducted additional experiments to investigate the effectiveness of using shallow layers of different models as a unified model for detection. The results, presented in Table~\ref{tab:table3}, confirm that the detection of Advp-MoblieNetV2 remains the most challenging among all the threat models' adversarial patches, as we previously discussed. In the absence of Advp-MoblieNetV2, it can be concluded that the first convolution layers of all models are suitable for detection, with the F-score reaching at least 92.17\%. However, when considering Advp-MoblieNetV2, only the first convolution layers of ResNet-50 and MobileNet-V2 are additional options as unified models for detection, with an F-score of at least 80.91\%. Combining the results from Table~\ref{tab:table2} and Table~\ref{tab:table3}, we can state that the second layer of VGG-16 is the best-performing unified model for detecting all adversarial patches trained from different threat models. The F-score achieved by this model is at least 97.42\%, surpassing the previous state-of-the-art performance achieved by LanCe~\cite{xu2020lance}. LanCe attained an accuracy of 91\% but did not consider the possibility of falsely classifying clean images as attacked.

\textbf{Interpretation of Results:} The optimal choice obtained from the experimental results may be attributed to the fact that VGG-16 is the most vulnerable model among all the threat models, as shown in Table~\ref{tab:table1}. This vulnerability allows patches trained by other threat models to possess some level of transferability to attack VGG-16. As a result, the shallow layers of VGG-16 demonstrate sensitivity to all patches and exhibit the capability to capture pertinent features that indicate the presence of adversarial patches.

%The reason for this result may be that the VGG-16 is the most vulnerable among all the threat models, so all patches trained by other models have some level of transferability to attack VGG-16. As a result, the shallow layers of VGG-16 are sensitive to all patches and have the ability to capture relevant features indicative of adversarial patches.

%This happens may because from the adversarial attacks training, we can see the VGG-16 is the most vulnerable model

\input{_tab/tab3}
\input{_tab/table5_v2}

%\subsection{Memory and Operation Complexity}
% 将以上各种patch，换其他模型的浅层进行检测, 列出实验结果和图，以及不同的threshold值
% 确定哪个模型的浅层更适合作为统一的检测模型
% 这个确定的过程中，不应该只看实验结果，在实验结果差不多的情况下，应选择浅层结构更简单的模型
% 选择的指导建议
% 浅层结构的复杂度评估：
% 1.计算单元的数量 
% 2.计算过程中需要store并transfer的中间结果数量 
% 3.MADD,FLOPS
% 1.可以找到模型
% 2.实验指导意义

%In order to guide the layer and model selection for patch detection, we analyzed the information of each model shallow layer, as shown in Table~\ref{tab:table4}.

%\input{_tab/tab4}


\subsection{Computational Cost}
In this section, we aim to benchmark the computational cost introduced by our proposed method against those incurred by previous methods. 
% The computational cost comparsion will not include the inference of CNNs as each method have. 
The computational cost directly influences the speed and efficiency of these methods. Our comparisons will focus on two aspects and all comparisons will conduct with different deep CNN models. 
% Note that the comparison only considers the cost introduced by these methods，excluding the original neural network computation.

Firstly, we evaluate the preliminary computations required before the methods can be deployed, 
% we need consider the preparatory work required before the deployment of methods, 
including the calculation of thresholds in ours and LanCe's, and verify process (calculation of FNC and IFNR) in Yu's. 
LanCe's detection process comprises three stages: 2D Fast Fourier Transform (2D-FFT), Class Activation Mapping (CAM) and Jaccard Similarity Coefﬁcient (JSC) calculations. Given C classes with N examples each, each stage executes $ CN$ times to acquire the necessary thresholds.
The CAM calculation involves ADD operations on the final feature map (FFM). 
% of size $k\times h\times w$. 
For an image of dimensions $H\times W$, the 2D-FFT calculation involves $(HW\log(W) + HW\log(H))$ multiplications and equivalent ADD operations. The JSC calculation requires logical AND or OR operations executed $hw\log(hw)$ times.
In Yu's methodology, the calculation of the IFNR for each pair of adversarial and clean images involves generating norm maps from the final feature maps, supplemented by four SUB/ADD and comparison operations within these map dimensions. Additionally, they introduce FNC layers to the feature maps of each cascaded module (e.g. Convolution block for VGG-16). For simplicity in comparison, we assume they add the FNC layer only to the first cascaded module.
% Generating the norm map for a $k\times h\times w$ dimensional feature map requires $khw$ multiplications and an equal number of ADD operations. 
Our method, however, focuses computationally on generating the attention map from the feature map of the second convolution layer, specifically the first convolution block of VGG-16. We then identify the maximum value within this attention map.

% Indeed, we are assuming that the number of examples N, used in our method to compute thresholds and in Yu's method to calculate IFNRs, is the same. This assumption is based on the equal number of examples used in LanCe to calculate thresholds for each class. 
% \input{_tab/table5_v2}

The comparison of computational cost during the threshold calculation and verify stage of these methods is presented in Table~\ref{tab:table5}. The results suggest that our method demands considerably fewer computational resources during this stage than the LanCe and Yu approaches. More specifically, ours involves only ADD/SUB and comparison operations, which are less complex at the hardware level and less demanding in processing power than the multiplication operations necessitated by the other two methods.

% Because multiplication requires a series of shift and ADD operations, while ADD operation can usually be completed in one processor cycle.
% Thus, our approach provides a more computationally efficient solution for practical applications.

% \input{_tab/table6}

% \input{_tab/table7}

Secondly, we assess the computational costs during the actual implementation stages of these methods. During this phase, Yu's method emphasizes on the computation of FNC layers, while LanCe executes the same three steps as in its former stage for each sample. The comparison of this stage is illustrated in Table~\ref{tab:table5}. Our method stands out by significantly reducing the computational burden, primarily by avoiding the expensive multiplication operations. Moreover, our method exhibits superior efficiency by requiring only a single register to store the threshold, a sharp contrast to LanCe's requirement of 1000 registers for multiple thresholds. This efficiency not only conserves memory space but also simplifies system implementation and minimizes overall complexity. 

% Table~\ref{tab:table7} provides a summary of the computational operations involved throughout all stages.

In conclusion, our method proves highly efficient due to its lower computational cost and reduced need for register storage, making it particularly suitable for deployment in resource-constrained environments, such as edge devices.

% our approach emerges as a highly efficient solution, particularly apt for deployment in resource-constrained settings, such as edge devices.
% As a result, our approach proves highly efficient and well-suited for deployment in resource-constrained environments, such as edge devices.



==> _his/4-Experiment_v3.tex <==
\section{Experiment and Evaluation}
The experiment details are presented in Fig.~\ref{fig:Fig5}. We perform a 4:6 stratified random sampling of the ImageNet dataset~\cite{russakovsky2015imagenet} to obtain the analysis dataset (40\%) and the test dataset (60\%). Half of the test dataset is randomly attacked to generate a balanced dataset of positive (attacked images) and negative (clean images) samples. Using the analysis dataset, we calculate the threshold $\Theta$ of $I_{r}$ indicators, which we utilized to detect the test dataset.

\subsection{Experiment Setup}
% 介绍模型的评价指标P,R,F
% 总的实验框架图，分为分析和测试两步Fig. 7.

\textbf{Evaluation Metric:} 
Unlike previous research, which evaluated detection models solely based on accuracy using only attacked images as input data, our approach is comprehensively evaluated using commonly used classifier metrics, including precision ($P$), recall ($R$), and F-score ($F$). These metrics require the model's input dataset to consist of both positive and negative samples, allowing us to account for the possibility of falsely classifying clean images as attacked.

\textbf{Detection Layer:} The shallow layers used to obtain $I_{r}$ indicators are taken from VGG-16, but other classic models such as ResNet-50, MobileNet-V3, and others can also be used. The selection of detector models and layers will be discussed in the Ablation Studies section.

\input{_tab/tab1_v2}

\textbf{Attacks Training:} We utilized the original adversarial patch attacks developed by Brown et al.~\cite{brown2017adversarial} to train diverse adversarial patches, which occupy only 6\% of the original image size, against several typical deep CNNs, respectively. We extracted a small sample of 2000 images from ImageNet to train these patches. As presented in Table~\ref{tab:table1}, the top-1 accuracy of the corresponding threat models was reduced to the range of 0.83\% to 33.98\% on Imagenet.



\subsection{Effectiveness of Detection} % Performance of Detection
% 简单介绍针对各种thread models 在Imagenet数据集训练的patch
% vgg16模型的浅层用于检测各种patch，列出实验结果和图，以及模型求出的参数：threshold值
% 实验结果可以和Lance中detection部分进行比较
% 说明在模型应对针对不同网络的patch时，检测层无需做出变更，甚至threshold值都不需要改变
%gpu cost 
From Table~\ref{tab:table1} we observe that adversarial patches cause varying degrees of Top-1 accuracy degradation in classical models, with VGG-16 being the most vulnerable to patch attacks, while MoblieNet-V2 is relatively robust and difficult to attack. We aim to build a unified model to detect all threat models' adversarial patches. 

\input{_tab/tab2}
% \input{_tab/tab3}

To accomplish this, we leverage the shallow layers of VGG16 as a unified model to derive the $I_{r}$ indicator and calculate $\Theta$. The detection results, as shown in Table~\ref{tab:table2}, reveal that the second convolutional layer of VGG-16 emerges as the optimal choice for the detection layer, i.e., utilizing the $I_{r}$ indicator, derived from the feature map after the first two layers, offers the best performance in attack detection. All attacked inputs can be correctly identified (R=100\%), and about 95\% of clean images are guaranteed not to be falsely identified as attacked (P$\approx$95\%), with an F-score of at least 97.42\%. The results also suggest that one of the adversarial patches, called Advp-MobileNetV2, which is trained on the robust MobileNet-V2, tends to be more aggressive and exhibits higher cross-model transferability, making it challenging to detect. In scenarios where the edge device is grappling with extreme resource constraints, deploying only the first layer of VGG-16 could still be a viable option. It retains an F-score of at least 87.91\%, even when subjected to the Advp-MoblieNetV2 attack.

% \input{_tab/tab2}
\input{_tab/tab3}

\textbf{Ablation Studies:} We conducted additional experiments to investigate the effectiveness of using shallow layers of different models as a unified model for detection. The results, presented in Table~\ref{tab:table3}, confirm that the detection of Advp-MoblieNetV2 remains the most challenging among all the threat models' adversarial patches, as we previously discussed. In the absence of Advp-MoblieNetV2, it can be concluded that the first convolution layers of all models are suitable for detection, with the F-score reaching at least 92.17\%. However, when considering Advp-MoblieNetV2, only the first convolution layers of ResNet-50 and MobileNet-V2 are additional options as unified models for detection, with an F-score of at least 80.91\%. Combining the results from Table~\ref{tab:table2} and Table~\ref{tab:table3}, we can state that the second layer of VGG-16 is the best-performing unified model for detecting all adversarial patches trained from different threat models. The F-score achieved by this model is at least 97.42\%, surpassing the previous state-of-the-art performance achieved by LanCe~\cite{xu2020lance}. LanCe attained an accuracy of 91\% but did not consider the possibility of falsely classifying clean images as attacked.

\textbf{Interpretation of Results:} The optimal choice obtained from the experimental results may be attributed to the fact that VGG-16 is the most vulnerable model among all the threat models, as shown in Table~\ref{tab:table1}. This vulnerability allows patches trained by other threat models to possess some level of transferability to attack VGG-16. As a result, the shallow layers of VGG-16 demonstrate sensitivity to all patches and exhibit the capability to capture pertinent features that indicate the presence of adversarial patches.

%The reason for this result may be that the VGG-16 is the most vulnerable among all the threat models, so all patches trained by other models have some level of transferability to attack VGG-16. As a result, the shallow layers of VGG-16 are sensitive to all patches and have the ability to capture relevant features indicative of adversarial patches.

%This happens may because from the adversarial attacks training, we can see the VGG-16 is the most vulnerable model


\input{_tab/table5_v2}

%\subsection{Memory and Operation Complexity}
% 将以上各种patch，换其他模型的浅层进行检测, 列出实验结果和图，以及不同的threshold值
% 确定哪个模型的浅层更适合作为统一的检测模型
% 这个确定的过程中，不应该只看实验结果，在实验结果差不多的情况下，应选择浅层结构更简单的模型
% 选择的指导建议
% 浅层结构的复杂度评估：
% 1.计算单元的数量 
% 2.计算过程中需要store并transfer的中间结果数量 
% 3.MADD,FLOPS
% 1.可以找到模型
% 2.实验指导意义
%In order to guide the layer and model selection for patch detection, we analyzed the information of each model shallow layer, as shown in Table~\ref{tab:table4}.
%\input{_tab/tab4}

\input{_tab/table8}
\subsection{Computational Cost}
In this section, we aim to benchmark the computational cost introduced by our proposed method against those incurred by previous methods. 
% The computational cost comparsion will not include the inference of CNNs as each method have. 
The computational cost directly influences the speed and efficiency of these methods. Our comparisons will focus on two aspects and all comparisons will conduct with different deep CNN models. 
% Note that the comparison only considers the cost introduced by these methods，excluding the original neural network computation.

Firstly, we evaluate the preliminary computations required before the methods can be deployed, 
% we need consider the preparatory work required before the deployment of methods, 
including the calculation of thresholds in ours and LanCe's, and verify process (calculation of FNC and IFNR) in Yu's. 
LanCe's detection process comprises three stages: 2D Fast Fourier Transform (2D-FFT), Class Activation Mapping (CAM) and Jaccard Similarity Coefﬁcient (JSC) calculations. Given C classes with N examples each, each stage executes $ CN$ times to acquire the necessary thresholds.
% The CAM calculation involves ADD operations on the final feature map (FFM). 
% of size $k\times h\times w$. 
% For an image of dimensions $H\times W$, the 2D-FFT calculation involves $(HW\log(W) + HW\log(H))$ multiplications and equivalent ADD operations. The JSC calculation requires logical AND or OR operations executed $hw\log(hw)$ times.
In Yu's approach, the computations comprise the FNC layers, introduced at each cascaded module (examples include introducing the FNC layer after each convolution block in VGG-16), and INFR, which necessitates calculating the L-2 norm of the feature map. To simplify comparison, we assume that the FNC layer is added only to the initial cascaded module.
% they calculate the INFR for each pair of adversarial and clean images that involve computing norm maps and introduce FNC layers to the feature maps of each cascaded module (e.g. Convolution block for VGG-16). For simplicity in comparison, we assume they add the FNC layer only to the first cascaded module.
% In Yu's methodology, the calculation of the IFNR for each pair of adversarial and clean images involves generating norm maps from the final feature maps, supplemented by four SUB/ADD and comparison operations within these map dimensions. Additionally, they introduce FNC layers to the feature maps of each cascaded module (e.g. Convolution block for VGG-16). For simplicity in comparison, we assume they add the FNC layer only to the first cascaded module.
% Generating the norm map for a $k\times h\times w$ dimensional feature map requires $khw$ multiplications and an equal number of ADD operations. 
Our method, however, focuses computationally on generating the attention map from the feature map of the second convolution layer, i.e., the first convolution block of VGG-16. We then identify the maximum value within this attention map.
% Indeed, we are assuming that the number of examples N, used in our method to compute thresholds and in Yu's method to calculate IFNRs, is the same. This assumption is based on the equal number of examples used in LanCe to calculate thresholds for each class. 
% \input{_tab/table5_v2}
% The comparison of computational cost during the threshold calculation and verify stage of these methods is presented in Table~\ref{tab:table5}. The results suggest that our method demands considerably fewer computational resources during this stage than the LanCe and Yu approaches. More specifically, ours involves only ADD/SUB and comparison operations, which are less complex at the hardware level and less demanding in processing power than the multiplication operations necessitated by the other two methods.
% Because multiplication requires a series of shift and ADD operations, while ADD operation can usually be completed in one processor cycle.
% Thus, our approach provides a more computationally efficient solution for practical applications.
% \input{_tab/table6}
% \input{_tab/table7}
Secondly, we assess the computational costs during the actual implementation stages of these methods. During this phase, Yu's method emphasizes the computation of FNC layers, while LanCe's and Ours execute the same steps as in the former stage for each sample.

The comparison is illustrated in Table~\ref{tab:table5}, where all computations mentioned above can be dissected into four basic types of hardware operations. Our method stands out by significantly reducing the computational burden, primarily by avoiding the expensive multiplication operations. Moreover, our method exhibits superior efficiency by requiring only a single register to store the threshold, a sharp contrast to LanCe's requirement of 1000 registers for multiple thresholds. This efficiency not only conserves memory space but also simplifies system implementation and minimizes overall complexity. 
Thereby, our method is particularly suitable for deployment in resource-constrained environments, such as edge devices.
% Table~\ref{tab:table7} provides a summary of the computational operations involved throughout all stages.
% Thereby, our method proves highly efficient due to its lower computational cost and reduced need for register storage, making it particularly suitable for deployment in resource-constrained environments, such as edge devices.

% our approach emerges as a highly efficient solution, particularly apt for deployment in resource-constrained settings, such as edge devices.
% As a result, our approach proves highly efficient and well-suited for deployment in resource-constrained environments, such as edge devices.

To demonstrate the superiority of our detection method in terms of latency and energy consumption, we executed our approach across three platforms: GPU (NVIDIA GeForce RTX 3090), CPU$^{1}$ (12th Gen Intel(R) Core(TM) i9-12900KF), and CPU$^{2}$ (Apple M2), the latter being the type of processor used in devices like the MacBook Air. CPU$^{2}$ has also been applied to mobile devices, such as the iPad Pro11. As a result, the experimental data corresponding to CPU$^{2}$ may be used as a close approximation to represent our method's performance on resource-constrained mobile devices.
Since previous approaches all incorporate full neural network models, their detection processes are invariably completed either simultaneously with or after the inference of the full model. Consequently, their latency and energy consumption are invariably equal to or greater than those associated with the full model's inference. To streamline the comparison, we contrasted our method directly with the full model. By demonstrating lower latency and energy consumption than the full model, our results indirectly assert that our approach is superior in efficiency to previous strategies. The comparative analysis was conducted across three distinct networks, whose shallow layers have previously been validated for strong detection performance. 

Table~\ref{tab:table8} illustrates the results, revealing that our method consistently shortens latency across all platforms, achieving speedup factors that range from 2.46x to 30.04x relative to the full models. Notably, CPU$^{2}$ achieves the highest speedup with MobileNet-V2 at 30.04x. Furthermore, energy savings are significant, ranging from 55.27\% to 97.05\%. CPU$^{1}$ demonstrates consistent energy efficiency, while MobileNet-V2 on CPU$^{2}$ reaches the peak saving at 97.05\%. These findings collectively confirm that our method markedly enhances both latency and energy efficiency across various platforms compared to previous approaches. Particularly, the performance on CPU$^{2}$ underscores our method's potential as a promising solution for real-time processing and energy-efficient applications in edge devices.





==> _his/4-Experiment_v4.tex <==
\section{Experiment and Evaluation}

\subsection{Experiment Setup}
Fig.~\ref{fig:Fig5} indicates the implementation detail of the proposed detection. 
The framework include two phases: analysis where the threshold $\Theta$ for a deployed DNN is calculated based on clean samples and evaluation which assesses the detection performance.

\textbf{Experiment Dataset:} A random sampling on the ImageNet dataset~\cite{russakovsky2015imagenet} yields 40\% for analysis and 60\% for testing. Half of the test data is attacked to create a balanced set of positive (attacked) and negative (clean) samples. The analysis dataset is used to calculate the threshold $\Theta$ of $I_{r}$ indicators for detecting the test dataset.

% A stratified random sampling on the ImageNet dataset~\cite{russakovsky2015imagenet} is performed to obtain 40\% analysis dataset and 60\% test dataset.
% Half of the test dataset is randomly attacked to generate a balanced dataset of positive (attacked) and negative (clean) samples.
% The analysis dataset is utilized to calculate the threshold $\Theta$ of $I_{r}$ indicators, which are utilize to detect the test dataset.

% 介绍模型的评价指标P,R,F
% 总的实验框架图，分为分析和测试两步Fig. 7.

\textbf{Evaluation Metric:} 
Unlike previous research that only evaluated accuracy of detection models with attacked images as input data, our approach comprehensively evaluates metrics including precision ($P$), recall ($R$), and F-score ($F$). 
Both positive and negative samples are included in the input dataset.
%These metrics require the model's input dataset to consist of both positive and negative samples, allowing us to account for the possibility of falsely classifying clean images as attacked.

\textbf{Detection Layer:} The shallow layers used to obtain $I_{r}$ indicators are from VGG-16, but other classic models such as ResNet-50, MobileNet-V3, etc. can also be utilized. The selection of detector models and layers are discussed in the below sections.

\input{_tab/tab1_v2}

\textbf{Attacks Training:} We utilize the adversarial patch attacks in~\cite{brown2017adversarial} to train diverse adversarial patches, which occupy only 6\% of the original image size and are utilized to attack several DNNs. 
A small sample of images (i.e., 4000) from ImageNet are leveraged to train these patches. As shown in Table~\ref{tab:table1}, the top-1 accuracy of the corresponding threat models on ImageNet can be reduced to 0.83\%.

\subsection{Effectiveness of Detection} % Performance of Detection
% 简单介绍针对各种thread models 在Imagenet数据集训练的patch
% vgg16模型的浅层用于检测各种patch，列出实验结果和图，以及模型求出的参数：threshold值
% 实验结果可以和Lance中detection部分进行比较
% 说明在模型应对针对不同网络的patch时，检测层无需做出变更，甚至threshold值都不需要改变
%gpu cost 
Table~\ref{tab:table1} shows that adversarial patches cause varying accuracy degradation on different DNNs. 
VGG-16 is the most vulnerable, while MoblieNet-V2 is relatively robust and difficult to attack.
In this work, We aim to build a unified model to successfully detect all threat models' adversarial patches. 

\input{_tab/tab2}
% \input{_tab/tab3}

To achieve this goal, we leverage shallow layers of VGG-16 as a unified model to derive the $I_{r}$ indicator and calculate $\Theta$. 
The detection results, as shown in Table~\ref{tab:table2}, reveal that the second convolutional layer of VGG-16 emerges as the optimal choice for the detection layer, i.e., utilizing the $I_{r}$ indicator, derived from the feature map after the first two layers, offers the best performance in attack detection. All attacked inputs can be correctly identified (R=100\%), and about 95\% of clean images are guaranteed not to be falsely identified as attacked (P$\approx$95\%), with an F-score of at least 97.42\%. 
The results also show that one of the adversarial patches, called Advp-MobileNetV2, which is trained on the robust MobileNet-V2, tends to be more aggressive and exhibits higher cross-model transferability, making it challenging to detect. 
As such, the detection model can be formed with only the first two convolution layers of VGG-16, which is lightweight and can be deployed in the resource limited edge devices.
The results also indicate that in scenarios where computing resource is extremely limited, deploying only the first layer is still possible with an F-score of at least 87.91\%, even when subjected to the Advp-MoblieNetV2 attack.

% \input{_tab/tab2}
\input{_tab/tab3}

%\textbf{Ablation Studies:} 
We also conducted experiments to investigate the effectiveness of using shallow layers of different models as a unified model for detection. 
% The results in Table~\ref{tab:table3} demonstrated that the first convolution layer of all models except the Advp-MoblieNetV2 is suitable to form the detection model, with the F-score reaching at least 92.17\%. 
The results in Table~\ref{tab:table3} demonstrated that without considering patch Advp-MoblieNetV2, the first convolution layers of all models are suitable for forming the detection model, achieving an F-score of at least 92.17\%.
Considering Advp-MoblieNetV2, only the first convolution layers of ResNet-50 and MobileNet-V2 are appropriate for constructing the detection model, achieving an F-score of at least 80.91\%.
% its first convolution layer is only suitable to form the unified detection model for ResNet-50 and MobileNet-V2 with an F-score of at least 80.91\%. 

Results from Table~\ref{tab:table2} and Table~\ref{tab:table3} demonstrate that the unified detection model formed by the first two convolution layers of VGG-16 has the best performance against all adversarial patches trained from different threat models. 
A F-score of at least 97.42\% is achieved, which is significantly higher than LanCe~\cite{xu2020lance} with a detection accuracy of 91\%.
%without considering the possibility of falsely classifying clean images as attacked. 

\textbf{Interpretation of Results:} The optimal choice obtained from the experimental results may be attributed to the fact that VGG-16 is the most vulnerable model among all the threat models, as shown in Table~\ref{tab:table1}. This vulnerability allows patches trained by other threat models to possess some level of transferability to attack VGG-16. As a result, the shallow layers of VGG-16 demonstrate sensitivity to all patches and exhibit the capability to capture pertinent features that indicate the presence of adversarial patches.


%The reason for this result may be that the VGG-16 is the most vulnerable among all the threat models, so all patches trained by other models have some level of transferability to attack VGG-16. As a result, the shallow layers of VGG-16 are sensitive to all patches and have the ability to capture relevant features indicative of adversarial patches.

%This happens may because from the adversarial attacks training, we can see the VGG-16 is the most vulnerable model


% \input{_tab/table5_v2}

%\subsection{Memory and Operation Complexity}
% 将以上各种patch，换其他模型的浅层进行检测, 列出实验结果和图，以及不同的threshold值
% 确定哪个模型的浅层更适合作为统一的检测模型
% 这个确定的过程中，不应该只看实验结果，在实验结果差不多的情况下，应选择浅层结构更简单的模型
% 选择的指导建议
% 浅层结构的复杂度评估：
% 1.计算单元的数量 
% 2.计算过程中需要store并transfer的中间结果数量 
% 3.MADD,FLOPS
% 1.可以找到模型
% 2.实验指导意义
%In order to guide the layer and model selection for patch detection, we analyzed the information of each model shallow layer, as shown in Table~\ref{tab:table4}.
%\input{_tab/tab4}

\input{_tab/table8}
\subsection{Computing Efficiency}
% In this section, we aim to benchmark the computational cost introduced by our proposed method against those incurred by previous methods. 
% The computational cost comparsion will not include the inference of CNNs as each method have. 
% The computational cost directly influences the speed and efficiency of these methods. Our comparisons will focus on two aspects and all comparisons will conduct with different deep CNN models. 
% Note that the comparison only considers the cost introduced by these methods，excluding the original neural network computation.

% Firstly, we evaluate the preliminary computations required before the methods can be deployed, 
% we need consider the preparatory work required before the deployment of methods, 
% including the calculation of thresholds in ours and LanCe's, and verify process (calculation of FNC and IFNR) in Yu's. 
% LanCe's detection process comprises three stages: 2D Fast Fourier Transform (2D-FFT), Class Activation Mapping (CAM) and Jaccard Similarity Coefﬁcient (JSC) calculations. Given C classes with N examples each, each stage executes $ CN$ times to acquire the necessary thresholds.
% The CAM calculation involves ADD operations on the final feature map (FFM). 
% of size $k\times h\times w$. 
% For an image of dimensions $H\times W$, the 2D-FFT calculation involves $(HW\log(W) + HW\log(H))$ multiplications and equivalent ADD operations. The JSC calculation requires logical AND or OR operations executed $hw\log(hw)$ times.
% In Yu's approach, the computations comprise the FNC layers, introduced at each cascaded module (examples include introducing the FNC layer after each convolution block in VGG-16), and INFR, which necessitates calculating the L-2 norm of the feature map. To simplify comparison, we assume that the FNC layer is added only to the initial cascaded module.
% they calculate the INFR for each pair of adversarial and clean images that involve computing norm maps and introduce FNC layers to the feature maps of each cascaded module (e.g. Convolution block for VGG-16). For simplicity in comparison, we assume they add the FNC layer only to the first cascaded module.
% In Yu's methodology, the calculation of the IFNR for each pair of adversarial and clean images involves generating norm maps from the final feature maps, supplemented by four SUB/ADD and comparison operations within these map dimensions. Additionally, they introduce FNC layers to the feature maps of each cascaded module (e.g. Convolution block for VGG-16). For simplicity in comparison, we assume they add the FNC layer only to the first cascaded module.
% Generating the norm map for a $k\times h\times w$ dimensional feature map requires $khw$ multiplications and an equal number of ADD operations. 
% Our method, however, focuses computationally on generating the attention map from the feature map of the second convolution layer, i.e., the first convolution block of VGG-16. We then identify the maximum value within this attention map.
% Indeed, we are assuming that the number of examples N, used in our method to compute thresholds and in Yu's method to calculate IFNRs, is the same. This assumption is based on the equal number of examples used in LanCe to calculate thresholds for each class. 
% \input{_tab/table5_v2}
% The comparison of computational cost during the threshold calculation and verify stage of these methods is presented in Table~\ref{tab:table5}. The results suggest that our method demands considerably fewer computational resources during this stage than the LanCe and Yu approaches. More specifically, ours involves only ADD/SUB and comparison operations, which are less complex at the hardware level and less demanding in processing power than the multiplication operations necessitated by the other two methods.
% Because multiplication requires a series of shift and ADD operations, while ADD operation can usually be completed in one processor cycle.
% Thus, our approach provides a more computationally efficient solution for practical applications.
% \input{_tab/table6}
% \input{_tab/table7}
% Secondly, we assess the computational costs during the actual implementation stages of these methods. During this phase, Yu's method emphasizes the computation of FNC layers, while LanCe's and Ours execute the same steps as in the former stage for each sample.

% The comparison is illustrated in Table~\ref{tab:table5}, where all computations mentioned above can be dissected into four basic types of hardware operations. Our method stands out by significantly reducing the computational burden, primarily by avoiding the expensive multiplication operations. Moreover, our method exhibits superior efficiency by requiring only a single register to store the threshold, a sharp contrast to LanCe's requirement of 1000 registers for multiple thresholds. This efficiency not only conserves memory space but also simplifies system implementation and minimizes overall complexity. 
% Thereby, our method is particularly suitable for deployment in resource-constrained environments, such as edge devices.
% Table~\ref{tab:table7} provides a summary of the computational operations involved throughout all stages.
% Thereby, our method proves highly efficient due to its lower computational cost and reduced need for register storage, making it particularly suitable for deployment in resource-constrained environments, such as edge devices.

% our approach emerges as a highly efficient solution, particularly apt for deployment in resource-constrained settings, such as edge devices.
% As a result, our approach proves highly efficient and well-suited for deployment in resource-constrained environments, such as edge devices.

The computing efficiency in speed and energy consumption of the proposed detection model is evaluated across three platforms: GPU (NVIDIA GeForce RTX 3090), CPU$^{1}$ (12th Gen Intel(R) Core(TM) i9-12900KF), and CPU$^{2}$ (Apple M2).
%To demonstrate the superiority of our detection method in terms of latency and energy consumption, we executed our approach across three platforms: GPU (NVIDIA GeForce RTX 3090), CPU$^{1}$ (12th Gen Intel(R) Core(TM) i9-12900KF), and CPU$^{2}$ (Apple M2), the latter being the type of processor used in devices like the MacBook Air. CPU$^{2}$ has also been applied to mobile devices, such as the iPad Pro11. As a result, the experimental data corresponding to CPU$^{2}$ may be used as a close approximation to represent our method's performance on resource-constrained mobile devices.
Since all the previous approaches incorporate full neural network models, their detection processes are invariably completed either simultaneously with or after the inference of the full model. %Consequently, their latency and energy consumption are invariably equal to or greater than those associated with the full model's inference. 
Therefore, we also compared the computing efficiency with detection using full models.
% To streamline the comparison, we contrasted our method directly with the full model. By demonstrating lower latency and energy consumption than the full model, our results indirectly assert that our approach is superior in efficiency to previous strategies. 
The comparative analysis is conducted across three DNNs, whose shallow layers have demonstrate high detection accuracy. 

Table~\ref{tab:table8} illustrates that the proposed lightweight detection model can significantly reduce latency across all the three platforms, achieving speedup range from 2.46$\times$ to 30.04$\times$. 
CPU$^{2}$ achieves the highest speedup with MobileNet-V2 at 30.04$\times$. 
Energy savings are significant, ranging from 55.27\% to 97.05\%. CPU$^{1}$ demonstrates consistent energy efficiency, while MobileNet-V2 on CPU$^{2}$ reaches the peak saving at 97.05\%. These findings show that the proposed method significantly enhances both latency and energy efficiency across various platforms compared to previous approaches. The performance on CPU$^{2}$ demonstrates that our method is particularly promising to be applied on edge devices.

Compared with previous approaches, our attention-based detection significantly reduces computational load by avoiding introducing costly multiplication operations.
The proposed method requires only a single register to store one threshold compared to LanCe's 1000 registers for 1000 thresholds~\cite{xu2020lance}, resulting in a substantial reduction in memory utilization.
The lightweight detection model can significantly reduce implementation and hardware design complexity, making it particularly suitable for resource-constrained environments.


==> _his/tab2_v1.tex <==
\begin{table}[h]
    \vspace{-2mm}
    \setlength{\abovecaptionskip}{1.4mm}
    \setlength{\belowcaptionskip}{-0.cm}
    % \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \small
    \caption{Detection Performance Comparison Using Different Shallow Layers of VGG-16 as Detection Layer}
    \centering
        \tabcolsep 5.5pt
    \begin{tabular}{l|c|cccc}
    \hline
        \multicolumn{2}{c|}{Layer} & \textbf{Conv1} & \textbf{Conv2} & Conv3 & Conv4 \\ \hline
        \multicolumn{2}{c|}{Threshold} & 1.55 & 4.48 & 2.91 & 7.59 \\ \hline
        \multirow{3}{*}{\tabincell{l}{AdvP\\-VGG16}} & P(\%) & 94.85 & 94.99 & 94.95 & 95.09 \\
        ~ & R(\%) & 100 & 100 & 100 & 100 \\
        ~ & F(\%) & 97.36 & 97.43 & 97.41 & 97.48 \\ \hline
        \multirow{3}{*}{\tabincell{l}{AdvP\\-ResNet50}}& P(\%) & 95.28 & 95.44 & 95.29 & 95.19 \\
        ~ & R(\%) & 100 & 100 & 100 & 100 \\
        ~ & F(\%) & 97.58 & 97.67 & 97.59 & 97.54 \\ \hline
        \multirow{3}{*}{\tabincell{l}{AdvP\\-MobileNetV2}} & P(\%) & 93.92 & 95.29 & 93.99 & 75.88 \\
        ~ & R(\%) & 82.63 & 100 & 83.35 & 16.04 \\
        ~ & F(\%) & 87.91 & 97.59 & 88.35 & 26.48 \\ \hline
        \multirow{3}{*}{\tabincell{l}{AdvP\\-InceptionV3}} & P(\%) & 95.14 & 95.32 & 95.12 & 94.92 \\
        ~ & R(\%) & 100 & 100 & 100 & 100 \\
        ~ & F(\%) & 97.51 & 97.60 & 97.50 & 97.40 \\ \hline
        \multirow{3}{*}{\tabincell{l}{AdvP\\-ResNet101}} & P(\%) & 94.94 & 95.44 & 95.12 & 95.01 \\
        ~ & R(\%) & 100 & 100 & 100 & 100 \\
        ~ & F(\%) & 97.41 & 97.67 & 97.50 & 97.44 \\
    \hline
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
        \item[] Conv\#n means cascade shallow layers from first Conv layer to the nth layer.
     \end{tablenotes}
    \vspace{-6mm}
    \label{tab:table2}
\end{table}

==> _his/tab3_v1.tex <==
\begin{table*}[b]
    \vspace{-3mm}
    \setlength{\abovecaptionskip}{1.4mm}
    \setlength{\belowcaptionskip}{-0.cm}
    % \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \small
    \caption{Patches Detection Results with Shallow Layers of Other Models}
    \centering
        \tabcolsep 9pt
    \begin{tabular}{l|c|cc|cc|cc|cc}
    \hline
        \multicolumn{2}{c|}{Model} & \multicolumn{2}{c|}{ResNet-50} & \multicolumn{2}{c|}{MobileNet-V2} & \multicolumn{2}{c|}{Inception-V3} & \multicolumn{2}{c}{ResNet-101} \\
        \multicolumn{2}{c|}{Layer} & \textbf{Conv1} & Conv2-1 & \textbf{Conv1} & Conv2 & Conv1 & Conv2 & Conv1 & Conv2-1 \\ \hline
        \multicolumn{2}{c|}{Threshold} & 11.08 & 1.41 & 2.81 & 7.41 & 1.11 & 1.03 & 10.08 & 1.22 \\ \hline
         \multirow{3}{*}{\tabincell{l}{AdvP\\-VGG16}} & P(\%) & 95.51 & 95.27 & 95.68 & 92.98 & 95.13 & 95.37 & 95.33 & 95.09 \\
        ~ & R(\%) & 100 & 99.98 & 100 & 65.43 & 100 & 100 & 100 & 99.76 \\
        ~ &F(\%) & 97.70 & 97.57 & 97.79 & 76.81 & 97.50 & 97.63 & 97.61 & 97.37 \\ \hline
        \multirow{3}{*}{\tabincell{l}{AdvP\\-ResNet50}} & P(\%) & 95.24 & 95.38 & 95.04 & 92.78 & 94.71 & 95.60 & 95.19 & 94.96 \\
        ~ &R(\%) & 100 & 100 & 92.64 & 65.2 & 100 & 100 & 100 & 100 \\
        ~ &F(\%) & 97.56 & 97.63 & 93.83 & 76.58 & 97.28 & 97.75 & 97.54 & 97.41 \\ \hline
        \textbf{\multirow{3}{*}{\tabincell{l}{AdvP\\-MobileNetV2}}} & P(\%) & 93.91 & 51.99 & 93.72 & 88.91 & 78.77 & 80.90 & 87.03 & 63.66 \\
        ~ &R(\%) & 74.24 & 4.87 & 71.18 & 40.13 & 20.31 & 20.33 & 32.96 & 9.75 \\
        ~ &F(\%) & 82.93 & 8.90 & 80.91 & 55.30 & 32.29 & 32.49 & 47.81 & 16.92 \\ \hline
        \multirow{3}{*}{\tabincell{l}{AdvP\\-InceptionV3}} & P(\%) & 95.42 & 95.49 & 95.64 & 94.20 & 94.82 & 95.13 & 94.98 & 94.82 \\
        ~ &R(\%) & 100 & 100 & 100 & 82.67 & 100 & 93.10 & 100 & 99.87 \\
        ~ &F(\%) & 97.66 & 97.69 & 97.77 & 88.06 & 97.34 & 94.10 & 97.42 & 97.28 \\ \hline
        \multirow{3}{*}{\tabincell{l}{AdvP\\-ResNet101}} & P(\%) & 95.06 & 95.58 & 95.58 & 90.20 & 94.37 & 94.89 & 95.40 & 94.64 \\
        ~ &R(\%) & 100 & 99.99 & 100 & 46.01 & 90.07 & 88.91 & 100 & 100 \\
        ~ &F(\%) & 97.47 & 97.73 & 97.74 & 60.94 & 92.17 & 91.80 & 97.64 & 97.25 \\
    \hline
    \end{tabular}
    \vspace{-3mm}
    \label{tab:table3}
\end{table*}

==> _tab/tab1.tex <==
\begin{table}[!b]
    \vspace{-3mm}
    \setlength{\abovecaptionskip}{1.4mm}
    \setlength{\belowcaptionskip}{-0.cm}
    \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \small
    \caption{Top-1 Acc (\%) on Deep CNNs Under Patches attacks}
    \centering
        \tabcolsep 3.5pt
    \begin{tabular}{l|ccccc}
    \hline
        \tabincell{c}{Patch\\Name}  &  \textbf{VGG-16} & \tabincell{c}{ResNet\\-50} & \tabincell{c}{MobileNet\\-V2} & \textbf{\tabincell{c}{Inception\\-V3}} & \tabincell{c}{ResNet\\-101} \\
    \hline
        Clean & 70.33 & 80.14 & 71.18 & 67.24 & 81.29 \\ \hline
        \tabincell{l}{AdvP\\-VGG16}  &  \textbf{0.83} & 77.54 & 68.48 & 57.97 & 78.88 \\ \hline
        \tabincell{l}{AdvP\\-ResNet50}  & 58.77 &  \textbf{14.70} & 67.71 & 54.26 & 77.87 \\ \hline
        \textbf{\tabincell{l}{AdvP\\-MobileNetV2}} & 52.13 & 75.18 &  \textbf{33.98} & 51.09 & 73.64 \\ \hline
        \tabincell{l}{AdvP\\-InceptionV3} & 50.18 & 76.47 & 67.31 &  \textbf{9.55} & 74.94 \\ \hline
        \tabincell{l}{AdvP\\-ResNet101} & 53.2 & 73.85 & 67.07 & 53.96 &  \textbf{7.42} \\
    \hline
    \end{tabular}
    \vspace{-5mm}
    \label{tab:table1}
\end{table}

==> _tab/tab4.tex <==
\begin{table}[!ht]
    \vspace{-3mm}
    \setlength{\abovecaptionskip}{1.4mm}
    \setlength{\belowcaptionskip}{-0.cm}
    \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \small
    \caption{Resource Consumption of Different Models}
    \centering
        \tabcolsep 4pt
    \begin{tabular}{l|c|cccc}
    \hline
        \multicolumn{2}{c|}{~} & \tabincell{c}{params\\(K)} & \tabincell{c}{memory\\(MB)} & \tabincell{c}{Madd\\(G)} & \tabincell{c}{Flops\\(G)} \\ \hline
        \multirow{3}{*}{VGG-16} & \textbf{Conv1} & \textbf{1.8} & \textbf{24.5} & \textbf{0.18} & \textbf{0.09} \\
        ~ & \textbf{+Conv2} & \textbf{38.7} & \textbf{52.1} & \textbf{3.9} & \textbf{2.0} \\
        ~ & Full & 138,400 & 109.4 & 31.0 & 15.5 \\ \hline
        \multirow{2}{*}{ResNet-50} & \textbf{Conv1} & \textbf{9.5} & \textbf{9.59} & \textbf{0.2} & \textbf{0.1} \\
        ~ & Full & 25,600 & 109.7 & 8.2 & 4.1 \\ \hline
        \multirow{2}{*}{MobileNet-V2} & \textbf{Conv1} & \textbf{0.9} & \textbf{4.59} & \textbf{0.02} & \textbf{0.01} \\
        ~ & Full & 3,500 & 74.3 & 0.6 & 0.3 \\ \hline
        \multirow{2}{*}{Inception-V3} & Conv1 & 0.9 & 3 & 0.02 & 0.01 \\
        ~ & Full & 23,800 & 36.7 & 5.7 & 2.9 \\ \hline
        \multirow{2}{*}{ResNet-101} & Conv1 & 9.5 & 9.95 & 0.2 & 0.1 \\
        ~ & Full & 44,500 & 161.8 & 15.7 & 7.8 \\
    \hline
    \end{tabular}
    \vspace{-3mm}
    \label{tab:table4}
\end{table}

==> _tab/table5.tex <==
\begin{table}[h]
    % \vspace{-3mm}
    \setlength{\abovecaptionskip}{1.4mm}
    \setlength{\belowcaptionskip}{-0.cm}
    \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \small
    \caption{Comparison of Computational Cost During the Preparatory Stage.} 
    \centering
        \tabcolsep 2pt
    \begin{tabular}{l|c|cccc}
    \hline
    Method & Model & ADD/SUB & Multiplications & AND/OR & Comparison \\ \hline
    LanCe & \multirow{3}{*}{VGG-16} & N*808.57G & N*783.48G & N*550K & --- \\ \cline{1-1} \cline{3-6}
    Yu  & & N*903.17K & N*853K & --- &N*827.91K  \\ \cline{1-1} \cline{3-6}
    ours & & N*802.82K & --- & --- & N*802.82K\\ \hline
    LanCe & \multirow{3}{*}{ResNet-50} & N*883.84G & N*783.48G & N*550K & --- \\ \cline{1-1} \cline{3-6}
    Yu  & & N*602.11K & N*401.41K & --- &N*301.06K  \\ \cline{1-1} \cline{3-6}
    ours & & N*200.7K & --- & --- & N*200.7K\\ \hline
    LanCe & \multirow{3}{*}{\tabincell{c}{MobileNet\\-V2}} & N*846.2G & N*783.48G & N*550K & --- \\ \cline{1-1} \cline{3-6}
    Yu  & & N*652.29K & N*526.85K & --- &N*464.13.06K  \\ \cline{1-1} \cline{3-6}
    ours & & N*401.41K & --- & --- & N*401.41K\\
    \hline
    \end{tabular}
    \vspace{-3mm}
    \label{tab:table5}
\end{table}

==> _tab/table5_v2.tex <==
\begin{table*}[t]
    \vspace{3mm}
    \setlength{\abovecaptionskip}{1.4mm}
    \setlength{\belowcaptionskip}{-0.cm}
    % \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \small
    \begin{threeparttable}
    \caption{Comparison of Computational Cost.$\dagger$} 
    \centering
        \tabcolsep 2pt
    \begin{tabular}{l|c|cccc|ccccc}
    \hline
    \multirow{2}{*}{Method} & \multirow{2}{*}{Model} & \multicolumn{4}{c|}{Pre-implementation Stage $\divideontimes$} & \multicolumn{4}{c}{Implementation stage} \\ \cline{3-11}
    ~& ~ & ADD/SUB & Multiplications & AND/OR & Comparison & ADD/SUB & Multiplications & AND/OR & Comparison & \tabincell{l}{Registers$\ddagger$} \\ \hline
    LanCe & \multirow{3}{*}{VGG-16} & N*808.57G & N*783.48G & N*550K & --- & 808.57K & 783.48K & 550 & --- & 1000 \\ \cline{1-1}
    Yu  & & N*903.17K & N*853K & --- & N*827.91K & 802.82K & 802.82K & --- & 802.82K & --- \\ \cline{1-1}
    ours & & N*802.82K & --- & --- & N*802.82K & 802.82K & --- & --- & 802.82K & 1 \\ \hline \hline
    LanCe & \multirow{3}{*}{ResNet-50} & N*883.84G & N*783.48G & N*550K & --- & 883.84k & 783.48k & 550 & --- & 1000 \\ \cline{1-1}
    Yu  & & N*602.11K & N*401.41K & --- & N*301.06K & 200.7K & 200.7K & --- & 200.7K & --- \\ \cline{1-1}
    ours & & N*200.7K & --- & --- & N*200.7K & 200.7K & --- & --- & 200.7K & 1\\ \hline \hline
    LanCe & \multirow{3}{*}{\tabincell{c}{MobileNet\\-V2}} & N*846.2G & N*783.48G & N*550K & --- & 846.2k & 783.48k & 550 & ---& 1000\\ \cline{1-1}
    Yu  & & N*652.29K & N*526.85K & --- &N*464.13.06K & 401.41K & 401.41K & --- &401.41K & --- \\ \cline{1-1}
    ours & & N*401.41K & --- & --- & N*401.41K & 401.41K & --- & --- & 401.41K & 1\\
    \hline
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
        \item[] $\dagger$ The comparison only considers the cost introduced by these methods, excluding the original model's.
        \item[] $\divideontimes$ Pre-implementation Stage includes threshold computation and method verification. \quad $\ddagger$ Only registers used for storing thresholds are counted here.
        \item[] --- represents not required.  \quad
        N represents the samples required for each threshold calculation.
     \end{tablenotes}
    \vspace{-2mm}
    \label{tab:table5}
    \end{threeparttable}
\end{table*}

==> _tab/table6.tex <==
\begin{table}[h]
    % \vspace{-3mm}
    \setlength{\abovecaptionskip}{1.4mm}
    \setlength{\belowcaptionskip}{-0.cm}
    \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \small
    \caption{Comparison of Computational Cost During the Detection stage.}
    \centering
        \tabcolsep 2.5pt
    \begin{tabular}{l|c|cccc}
    \hline
    Method & Model & ADD/SUB & Multiplications & AND/OR & Comparison \\ \hline
    LanCe & \multirow{3}{*}{VGG-16} & 808.57K & 783.48K & 550 & --- \\ \cline{1-1} \cline{3-6}
    Yu  & & 802.82K & 802.82K & --- &802.82K  \\ \cline{1-1} \cline{3-6}
    ours & & 802.82K & --- & --- & 802.82K\\ \hline
    LanCe & \multirow{3}{*}{ResNet-50} & 883.84k & 783.48k & 550 & --- \\ \cline{1-1} \cline{3-6}
    Yu  & & 200.7K & 200.7K & --- &200.7K  \\ \cline{1-1} \cline{3-6}
    ours & & 200.7K & --- & --- & 200.7K\\ \hline
    LanCe & \multirow{3}{*}{\tabincell{c}{MobileNet\\-V2}} & 846.2k & 783.48k & 550 & --- \\ \cline{1-1} \cline{3-6}
    Yu  & & 401.41K & 401.41K & --- &401.41K  \\ \cline{1-1} \cline{3-6}
    ours & & 401.41K & --- & --- & 401.41K\\
    \hline
    \end{tabular}
    \vspace{-3mm}
    \label{tab:table6}
\end{table}

==> _tab/table7.tex <==
\begin{table}[h]
    % \vspace{-3mm}
    \setlength{\abovecaptionskip}{1.4mm}
    \setlength{\belowcaptionskip}{-0.cm}
    \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \small
    \caption{Comparison of Involved Computational Operations.}
    \centering
        \tabcolsep 2.5pt
    \begin{tabular}{l|ccccc}
    \hline
        Method & ADD/SUB & Multiplications & AND/OR & Comparison & No. of thresholds \\
    \hline
        LanCe & ✓ & ✓ & ✓ & ✕ & 1000 \\ \hline
        Yu & ✓ & ✓ & ✕ & ✓ & 1 \\ \hline
        ours & ✓ & ✕ & ✕ & ✓ & 1 \\ \hline
    \end{tabular}
    \vspace{-5mm}
    \label{tab:table7}
\end{table}
